Clustered and Triggered Star Formation in W5: Observations with Spitzer

We present images and initial results from our extensive Spitzer Space Telescope imaging survey of the W5 H II region with the Infrared Array Camera (IRAC) and Multiband Imaging Photometer for Spitzer (MIPS). We detect dense clusters of stars, centered on the O stars: HD 18326, BD +60 586, HD 17505 and HD 17520. At 24 microns substantial extended emission is visible, presumably from heated dust grains that survive in the strongly ionizing environment of the H {\sc ii} region. With photometry of more than 18000 point sources, we analyze the clustering properties of objects classified as young stars by their IR spectral energy distributions (a total of 2064 sources) across the region using a minimal-spanning-tree algorithm. We find ~40--70% of infrared excess sources belong to clusters with >10 members. We find that within the evacuated cavities of the H II regions that make up W5, the ratio of Class II to Class I sources is ~7 times higher than for objects coincident with molecular gas as traced by 12CO emission and near-IR extinction maps. We attribute this contrast to an age difference between the two locations, and postulate that at least two distinct generations of star formation are visible across W5. Our preliminary analysis shows that triggering is a plausible mechanism to explain the multiple generations of star formation in W5, and merits further investigation.

==> tab6.tex <==
\begin{deluxetable}{lcccccccccccc}
\tabletypesize{\scriptsize}
\rotate
\tablenum{6}
\tablewidth{0pt}
\tablecaption{W5 Extragalactic Sources}
\tablehead{\colhead{ } & \colhead{RA} & \colhead{Dec} & \colhead{$J$} & \colhead{$H$} & \colhead{$K_S$} & \colhead{$[3.6]$} & \colhead{$[4.5]$} & \colhead{$[5.8]$} & \colhead{$[8.0]$} & \colhead{$[24]$} & \colhead{ } & \colhead{ } \\
\colhead{ID} & \colhead{(deg)} & \colhead{(deg)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{Type\tablenotemark{a}} & \colhead{P(YSO)\tablenotemark{b}}}
\startdata 
g1 & 41.176602 & 60.672605 & \nodata & \nodata & \nodata & 15.52(03) & 14.62(03) & 14.71(17) & 13.28(18) & \nodata & PAH & 0.00 \\
g2 & 41.189968 & 60.652874 & \nodata & \nodata & \nodata & 15.17(03) & 14.48(04) & 14.07(11) & 13.02(11) & \nodata & AGN & 0.28 \\
g3 & 41.190158 & 60.586695 & 17.00(19) & \nodata & 15.24(14) & 14.04(01) & 13.65(02) & 12.98(06) & 11.99(07) & \nodata & AGN & 0.22 \\
g4 & 41.242231 & 60.703623 & \nodata & \nodata & \nodata & 14.72(03) & 13.85(04) & 13.31(12) & 12.19(17) & \nodata & AGN & 0.05 \\
g5 & 41.245464 & 60.736165 & \nodata & \nodata & \nodata & 14.71(03) & 13.93(03) & 13.35(08) & 12.38(07) & \nodata & AGN & 0.10 \\
g6 & 41.252453 & 60.541187 & \nodata & \nodata & \nodata & 14.53(03) & 13.97(02) & 13.48(07) & 12.37(06) & \nodata & AGN & 0.37 \\
g7 & 41.256135 & 60.465426 & 14.27(04) & 13.83(04) & 13.62(04) & 13.47(01) & 13.51(02) & 13.57(08) & 11.77(03) & \nodata & PAH & 0.02 \\
g8 & 41.274375 & 60.732626 & 16.90(17) & 16.23(24) & 15.34(15) & 14.65(03) & 14.15(03) & 13.71(12) & 11.95(08) & \nodata & PAH & 0.00 \\
g9 & 41.293823 & 60.525857 & 15.26(05) & 14.61(06) & 14.55(08) & 14.36(01) & 14.32(03) & 14.25(12) & 13.69(18) & \nodata & AGN & 0.63 \\
g10 & 41.294108 & 60.520992 & \nodata & \nodata & \nodata & 15.30(03) & 14.64(03) & 13.96(09) & 12.96(09) & \nodata & AGN & 0.40 \\
g11 & 41.358768 & 60.563170 & \nodata & \nodata & \nodata & 15.58(03) & 15.25(04) & 14.56(12) & 13.76(14) & \nodata & AGN & 0.09 \\
g12 & 41.363478 & 60.508246 & \nodata & \nodata & \nodata & 15.24(03) & 14.86(03) & 14.34(12) & 13.26(11) & \nodata & AGN & 0.33 \\
g13 & 41.364339 & 60.427455 & \nodata & \nodata & \nodata & 15.16(03) & 14.67(02) & 14.09(11) & 13.18(08) & \nodata & AGN & 0.53 \\
g14 & 41.373498 & 60.548281 & \nodata & \nodata & \nodata & 15.84(04) & 15.19(04) & 14.49(13) & 13.27(09) & \nodata & AGN & 0.08 \\
g15 & 41.376071 & 60.562656 & 14.75(04) & 14.37(06) & 14.30(07) & 14.19(01) & 14.12(02) & 13.95(08) & 13.60(15) & \nodata & AGN & 0.64 \\
g16 & 41.381116 & 60.438208 & \nodata & \nodata & \nodata & 15.08(02) & 14.81(03) & 14.49(16) & 13.40(15) & \nodata & AGN & 0.44 \\
g17 & 41.387989 & 60.392907 & \nodata & \nodata & \nodata & 14.63(03) & 14.15(02) & 13.69(09) & 12.54(07) & \nodata & AGN & 0.51 \\
g18 & 41.389071 & 60.432594 & 16.08(09) & 15.55(13) & 15.42(16) & 14.91(02) & 14.61(03) & 14.42(14) & 13.44(10) & \nodata & AGN & 0.57 \\
g19 & 41.395148 & 60.547845 & \nodata & \nodata & \nodata & 15.04(04) & 14.45(03) & 14.06(11) & 13.69(18) & \nodata & AGN & 0.61 \\
g20 & 41.422706 & 60.387304 & 16.69(15) & 15.68(14) & 15.17(14) & 14.92(02) & 14.67(03) & 14.29(10) & 13.49(14) & \nodata & AGN & 0.68 \\
g21 & 41.447555 & 60.362748 & \nodata & \nodata & \nodata & 15.44(04) & 15.07(04) & 14.50(15) & 13.35(08) & \nodata & AGN & 0.22 \\
g22 & 41.447715 & 60.430944 & \nodata & \nodata & \nodata & 15.85(05) & 15.33(06) & 14.65(18) & 13.65(15) & \nodata & AGN & 0.08 \\
g23 & 41.451989 & 60.363867 & \nodata & \nodata & \nodata & 14.81(02) & 14.36(03) & 14.28(12) & 13.64(11) & \nodata & AGN & 0.76 \\
g24 & 41.459651 & 60.572154 & 16.52(13) & 15.04(09) & 14.31(07) & 13.53(03) & 13.29(02) & 12.81(06) & 10.34(03) & 7.04(13) & PAH & 0.00 \\
g25 & 41.468191 & 60.363470 & \nodata & \nodata & \nodata & 14.38(01) & 13.77(01) & 12.92(04) & 11.89(04) & \nodata & AGN & 0.16 \\
g26 & 41.468493 & 60.730588 & \nodata & \nodata & \nodata & 15.42(04) & 14.68(04) & 14.01(10) & 12.62(11) & 8.94(11) & AGN & 0.04 \\
g27 & 41.474744 & 60.588493 & \nodata & \nodata & \nodata & 14.35(03) & 13.81(03) & 13.29(07) & 12.19(07) & 8.88(10) & AGN & 0.37 \\
g28 & 41.480840 & 60.400864 & \nodata & \nodata & \nodata & 15.85(05) & 15.72(06) & 14.90(19) & 14.10(15) & \nodata & AGN & 0.00 \\
g29 & 41.485185 & 60.571971 & \nodata & \nodata & \nodata & 15.57(05) & 15.16(07) & 14.57(16) & 13.16(14) & \nodata & AGN & 0.07 \\
g30 & 41.490581 & 60.330748 & 14.83(03) & 14.40(04) & 14.29(07) & 14.10(01) & 14.11(02) & 14.03(14) & 13.55(14) & \nodata & AGN & 0.44 \\
g31 & 41.491078 & 60.402708 & \nodata & \nodata & \nodata & 15.03(02) & 14.86(04) & 14.63(15) & 13.83(15) & \nodata & AGN & 0.56 \\
g32 & 41.493974 & 60.604043 & \nodata & \nodata & \nodata & 15.18(04) & 14.70(04) & 14.51(17) & 13.04(15) & \nodata & PAH & 0.00 \\
g33 & 41.496718 & 60.686982 & 16.55(11) & 15.65(14) & 15.06(14) & 14.95(03) & 14.70(04) & 14.30(14) & 13.36(13) & 9.77(34) & AGN & 0.31 \\
g34 & 41.497633 & 60.404724 & \nodata & \nodata & \nodata & 15.19(03) & 14.08(02) & 12.86(06) & 11.65(04) & \nodata & AGN & 0.04 \\
g35 & 41.500557 & 60.256846 & 15.21(05) & 14.46(06) & 14.25(06) & 14.03(01) & 14.15(02) & 13.61(10) & 13.57(15) & \nodata & AGN & 0.32 \\
g36 & 41.512880 & 60.561167 & \nodata & \nodata & \nodata & 15.27(03) & 14.75(04) & 14.14(11) & 13.18(08) & \nodata & AGN & 0.33 \\
g37 & 41.521110 & 60.660479 & \nodata & \nodata & 15.32(17) & 14.43(04) & 13.94(03) & 13.06(10) & 11.70(15) & \nodata & AGN & 0.05 \\
g38 & 41.522722 & 60.588366 & 17.10(18) & 15.96(18) & 15.13(13) & 14.59(02) & 14.08(02) & 13.58(05) & 12.46(04) & 10.16(32) & AGN & 0.42 \\
g39 & 41.526317 & 60.405494 & \nodata & \nodata & \nodata & 16.41(06) & 15.46(05) & 14.19(11) & 13.35(08) & \nodata & AGN & 0.01 \\
g40 & 41.536711 & 60.305998 & \nodata & \nodata & \nodata & 14.61(02) & 14.38(04) & 13.88(11) & 11.11(02) & \nodata & PAH & 0.00 \\
g41 & 41.537616 & 60.320414 & \nodata & \nodata & \nodata & 15.18(03) & 14.83(03) & 14.59(11) & 12.12(04) & \nodata & PAH & 0.00 \\
g42 & 41.539739 & 60.673764 & 16.22(09) & 15.18(09) & 14.65(09) & 14.19(02) & 14.19(03) & 13.92(12) & 12.73(19) & \nodata & PAH & 0.00 \\
g43 & 41.540225 & 60.479553 & 15.66(06) & 14.90(08) & 14.58(08) & 14.45(02) & 14.38(02) & 14.02(09) & 13.84(13) & \nodata & AGN & 0.36 \\
g44 & 41.544504 & 60.270013 & 16.86(16) & 16.03(22) & 15.22(14) & 14.25(03) & 13.88(03) & 13.47(09) & 12.24(07) & \nodata & AGN & 0.22 \\
g45 & 41.552815 & 60.645693 & \nodata & \nodata & \nodata & 15.37(03) & 14.92(03) & 13.99(11) & 12.77(07) & 9.56(10) & AGN & 0.04 \\
g46 & 41.610699 & 60.568779 & \nodata & \nodata & \nodata & 16.01(10) & 14.78(04) & 14.32(17) & 13.38(13) & \nodata & AGN & 0.30 \\
g47 & 41.620994 & 60.433643 & 15.32(05) & 14.75(06) & 14.47(07) & 14.20(01) & 14.16(02) & 13.97(08) & 13.61(14) & \nodata & AGN & 0.36 \\
g48 & 41.625858 & 60.222037 & \nodata & \nodata & \nodata & 14.66(03) & 13.76(02) & 13.02(09) & 11.89(17) & \nodata & AGN & 0.08 \\
g49 & 41.630725 & 60.745397 & 16.45(10) & 15.77(14) & 15.23(14) & 14.67(02) & 14.24(02) & 13.63(06) & 12.85(07) & 9.80(12) & AGN & 0.28 \\
g50 & 41.641708 & 60.092141 & \nodata & \nodata & \nodata & 16.46(07) & 14.92(04) & 13.54(06) & 12.37(05) & \nodata & AGN & 0.02 \\
g51 & 41.657626 & 60.147166 & \nodata & \nodata & \nodata & 15.28(04) & 14.74(03) & 14.10(15) & 12.87(20) & \nodata & AGN & 0.14 \\
g52 & 41.657710 & 60.316869 & \nodata & \nodata & \nodata & 16.50(06) & 15.50(04) & 14.55(16) & 13.08(09) & 8.94(09) & AGN & 0.00 \\
g53 & 41.666763 & 60.147449 & \nodata & \nodata & \nodata & 15.64(06) & 14.73(03) & 13.66(08) & 12.86(08) & \nodata & AGN & 0.14 \\
g54 & 41.668591 & 60.138829 & \nodata & \nodata & \nodata & 14.96(03) & 14.20(03) & 13.51(08) & 12.68(10) & \nodata & AGN & 0.42 \\
g55 & 41.669506 & 60.141360 & \nodata & \nodata & \nodata & 15.15(04) & 13.91(02) & 12.99(06) & 12.13(06) & \nodata & AGN & 0.14 \\
g56 & 41.684232 & 60.158713 & \nodata & \nodata & \nodata & 15.41(03) & 14.53(02) & 13.88(09) & 13.29(14) & 8.31(13) & AGN & 0.39 \\
g57 & 41.747794 & 60.036148 & \nodata & \nodata & \nodata & 15.53(04) & 15.18(05) & 14.92(16) & 12.53(05) & 9.36(14) & PAH & 0.00 \\
g58 & 41.757899 & 59.758831 & 14.53(05) & 13.79(07) & 13.47(06) & 12.86(01) & 12.81(02) & 11.75(02) & 10.10(03) & \nodata & PAH & 0.00 \\
g59 & 41.759091 & 59.653787 & 14.26(04) & 13.89(04) & 13.64(04) & 13.59(01) & 13.56(02) & 13.51(08) & 12.43(08) & \nodata & PAH & 0.00 \\
g60 & 41.762854 & 60.575313 & \nodata & \nodata & \nodata & 14.67(04) & 14.27(03) & 13.72(08) & 12.81(15) & \nodata & AGN & 0.28 \\
g61 & 41.775494 & 60.965509 & \nodata & 14.35(05) & \nodata & 14.17(01) & 14.24(03) & 14.23(15) & 12.62(12) & \nodata & PAH & 0.00 \\
g62 & 41.785849 & 59.893920 & \nodata & 15.69(15) & 15.08(14) & 14.23(02) & 13.76(01) & 13.23(09) & 12.28(05) & \nodata & AGN & 0.25 \\
g63 & 41.790986 & 59.848820 & \nodata & \nodata & \nodata & 14.93(02) & 14.47(03) & 13.94(12) & 13.11(11) & \nodata & AGN & 0.28 \\
g64 & 41.792119 & 59.607302 & 15.01(04) & 14.39(04) & 14.31(07) & 14.22(01) & 14.22(03) & 14.24(14) & 12.97(08) & \nodata & PAH & 0.00 \\
g65 & 41.792674 & 59.706862 & \nodata & \nodata & \nodata & 16.05(09) & 15.03(05) & 14.20(10) & 13.00(08) & \nodata & AGN & 0.02 \\
g66 & 41.797205 & 60.796924 & \nodata & \nodata & \nodata & 15.06(03) & 14.74(03) & 14.11(11) & 11.69(04) & 7.36(06) & PAH & 0.00 \\
g67 & 41.814041 & 59.962980 & \nodata & \nodata & \nodata & 15.52(04) & 15.08(04) & 14.66(14) & 13.58(13) & \nodata & AGN & 0.14 \\
g68 & 41.815787 & 60.105112 & \nodata & \nodata & \nodata & 14.97(04) & 14.67(04) & 14.11(15) & 12.86(06) & 8.91(07) & AGN & 0.08 \\
g69 & 41.829675 & 59.779120 & 14.21(04) & 13.87(05) & 13.79(05) & 13.66(01) & 13.59(02) & 13.68(12) & 12.30(04) & \nodata & PAH & 0.00 \\
g70 & 41.852749 & 60.738867 & 15.03(03) & 14.30(04) & 13.93(04) & 13.80(01) & 13.80(01) & 13.27(09) & 12.30(09) & \nodata & AGN & 0.32 \\
g71 & 41.853848 & 59.824166 & 13.84(03) & 13.30(03) & 13.13(03) & 13.14(01) & 13.13(01) & 13.11(06) & 12.07(04) & \nodata & PAH & 0.00 \\
g72 & 41.859214 & 59.525512 & \nodata & \nodata & \nodata & 16.39(09) & 15.51(06) & 14.67(20) & 13.28(15) & \nodata & AGN & 0.00 \\
g73 & 41.862314 & 60.108929 & 15.62(06) & 14.71(06) & 14.57(08) & 14.33(02) & 14.35(02) & 14.24(11) & 13.65(19) & \nodata & AGN & 0.37 \\
g74 & 41.873343 & 60.027913 & \nodata & \nodata & \nodata & 14.69(01) & 14.07(02) & 13.57(05) & 12.22(04) & 8.64(06) & AGN & 0.09 \\
g75 & 41.875001 & 61.016441 & \nodata & \nodata & 15.28(14) & 14.46(02) & 14.11(02) & 13.44(07) & 12.66(11) & \nodata & AGN & 0.36 \\
g76 & 41.876964 & 60.125964 & 15.51(05) & 15.03(07) & 14.70(09) & 14.64(02) & 14.65(03) & 14.25(11) & 13.79(17) & \nodata & AGN & 0.34 \\
g77 & 41.885034 & 60.584807 & 15.19(05) & 14.60(08) & 14.52(09) & 14.28(07) & 14.37(07) & 13.59(12) & 12.65(16) & \nodata & AGN & 0.05 \\
g78 & 41.902305 & 60.542116 & \nodata & \nodata & \nodata & 15.71(04) & 14.68(03) & 13.22(08) & 12.36(07) & \nodata & AGN & 0.02 \\
g79 & 41.904684 & 59.829937 & 16.82(16) & 15.88(14) & 15.65(22) & 14.46(03) & 13.89(03) & 13.40(08) & 12.32(05) & 8.10(06) & AGN & 0.21 \\
g80 & 41.924941 & 59.997657 & \nodata & \nodata & \nodata & 15.86(04) & 14.88(03) & 13.92(08) & 12.89(06) & 9.45(14) & AGN & 0.07 \\
g81 & 41.928655 & 60.335111 & \nodata & \nodata & \nodata & 16.36(06) & 15.41(04) & 14.21(09) & 13.23(11) & \nodata & AGN & 0.01 \\
g82 & 41.933119 & 59.630765 & \nodata & \nodata & \nodata & 14.55(01) & 14.29(03) & 13.90(09) & 11.77(05) & 9.01(14) & PAH & 0.00 \\
g83 & 41.937119 & 59.902566 & 15.45(05) & 15.06(08) & 14.65(09) & 14.77(02) & 14.71(03) & 14.55(11) & 14.15(15) & \nodata & AGN & 0.34 \\
g84 & 41.938327 & 59.612106 & 14.19(03) & 13.86(04) & 13.83(04) & 13.71(01) & 13.78(02) & 13.73(10) & 12.40(04) & \nodata & PAH & 0.35 \\
g85 & 41.940526 & 60.098047 & \nodata & \nodata & \nodata & 14.79(03) & 14.45(04) & 14.08(12) & 11.53(06) & 8.35(05) & PAH & 0.00 \\
g86 & 41.946352 & 60.518664 & \nodata & \nodata & \nodata & 15.77(07) & 14.93(03) & 13.79(09) & 12.35(13) & \nodata & AGN & 0.01 \\
g87 & 41.967518 & 60.883834 & \nodata & \nodata & \nodata & 15.77(09) & 14.66(07) & 13.66(12) & 12.70(18) & \nodata & AGN & 0.02 \\
g88 & 41.973799 & 60.309480 & \nodata & \nodata & \nodata & 16.02(05) & 15.01(04) & 13.82(08) & 12.72(09) & \nodata & AGN & 0.01 \\
g89 & 41.974793 & 60.029371 & \nodata & \nodata & \nodata & 15.59(04) & 15.01(04) & 14.46(15) & 12.58(07) & 9.07(07) & PAH & 0.00 \\
g90 & 41.976336 & 59.842646 & \nodata & \nodata & \nodata & 14.96(02) & 13.85(02) & 12.79(03) & 11.60(02) & 8.27(04) & AGN & 0.02 \\
g91 & 41.978731 & 59.987604 & 15.22(04) & 14.63(06) & 14.34(07) & 14.26(01) & 14.26(02) & 14.27(11) & 13.76(12) & \nodata & AGN & 0.38 \\
g92 & 41.982398 & 59.983923 & \nodata & \nodata & \nodata & 15.02(02) & 14.12(02) & 13.25(04) & 12.34(04) & 8.27(05) & AGN & 0.09 \\
g93 & 41.985714 & 61.003514 & \nodata & \nodata & 15.20(12) & 13.91(02) & 13.24(02) & 13.62(10) & 12.36(12) & \nodata & PAH & 0.00 \\
g94 & 42.015059 & 61.028383 & \nodata & \nodata & \nodata & 14.87(03) & 13.88(02) & 12.72(05) & 11.90(10) & \nodata & AGN & 0.09 \\
g95 & 42.019505 & 60.512786 & \nodata & \nodata & \nodata & 15.33(03) & 14.61(03) & 14.48(16) & 12.27(11) & 9.90(48) & PAH & 0.00 \\
g96 & 42.025943 & 60.784386 & 14.78(03) & 13.94(03) & 13.82(04) & 13.55(01) & 13.55(01) & 12.92(07) & 11.67(12) & \nodata & PAH & 0.00 \\
g97 & 42.029451 & 60.795876 & \nodata & \nodata & \nodata & 15.08(04) & 14.04(02) & 13.28(06) & 12.56(14) & 8.57(12) & AGN & 0.36 \\
g98 & 42.030617 & 59.795858 & \nodata & \nodata & \nodata & 14.99(02) & 14.13(01) & 13.31(05) & 12.20(04) & 8.83(07) & AGN & 0.09 \\
g99 & 42.048343 & 60.561998 & \nodata & \nodata & \nodata & 15.03(03) & 14.60(03) & 13.77(12) & 12.60(15) & \nodata & AGN & 0.09 \\
g100 & 42.075688 & 59.856577 & \nodata & \nodata & \nodata & 15.69(04) & 15.40(04) & 14.40(13) & 13.42(19) & 8.77(08) & AGN & 0.01 \\
g101 & 42.091906 & 59.615888 & 14.15(03) & 13.84(04) & 13.42(04) & 13.29(01) & 13.30(01) & 13.48(09) & 11.47(02) & \nodata & PAH & 0.00 \\
g102 & 42.117819 & 59.948725 & \nodata & \nodata & \nodata & 16.47(06) & 15.78(06) & 14.59(13) & 13.48(17) & \nodata & AGN & 0.00 \\
g103 & 42.122801 & 60.989678 & \nodata & 16.43(23) & 15.31(14) & 14.44(02) & 14.03(02) & 13.41(07) & 10.95(03) & 7.68(07) & PAH & 0.00 \\
g104 & 42.129663 & 60.516176 & \nodata & \nodata & \nodata & 15.67(05) & 14.73(03) & 14.04(13) & 12.68(12) & \nodata & AGN & 0.04 \\
g105 & 42.152678 & 60.413658 & 15.88(07) & 15.46(11) & 15.02(11) & 14.95(02) & 14.90(04) & 14.31(13) & 12.95(17) & \nodata & PAH & 0.00 \\
g106 & 42.155786 & 59.727590 & \nodata & \nodata & \nodata & 15.56(05) & 15.05(04) & 14.19(09) & 13.57(10) & 9.83(13) & AGN & 0.12 \\
g107 & 42.162288 & 59.763781 & \nodata & \nodata & \nodata & 16.75(07) & 15.79(06) & 14.56(15) & 13.41(17) & 9.98(16) & AGN & 0.00 \\
g108 & 42.168940 & 59.591721 & 14.35(04) & 13.98(04) & 13.70(04) & 13.55(01) & 13.53(01) & 13.84(09) & 12.75(08) & \nodata & PAH & 0.25 \\
g109 & 42.177878 & 59.680044 & 15.08(04) & 14.59(06) & 14.44(08) & 14.30(01) & 14.24(02) & 14.29(09) & 13.63(09) & \nodata & AGN & 0.37 \\
g110 & 42.183824 & 59.850063 & \nodata & \nodata & \nodata & 14.70(02) & 14.23(02) & 13.85(07) & 13.70(12) & \nodata & AGN & 0.37 \\
g111 & 42.189565 & 60.529727 & \nodata & \nodata & \nodata & 15.77(16) & 15.79(20) & 13.07(14) & 11.34(15) & \nodata & PAH & 0.29 \\
g112 & 42.191226 & 60.346590 & 15.77(11) & 14.50(11) & 13.55(08) & 12.58(04) & 12.34(03) & 10.74(04) & 8.45(04) & 5.41(18) & PAH & 0.00 \\
g113 & 42.193737 & 59.895512 & 15.03(04) & 14.51(05) & 14.41(07) & 14.29(01) & 14.32(02) & 14.38(14) & 13.55(19) & \nodata & AGN & 0.08 \\
g114 & 42.212490 & 60.622102 & 17.13(21) & \nodata & 15.04(12) & 14.05(03) & 13.74(02) & 13.22(08) & 12.14(10) & \nodata & AGN & 0.19 \\
g115 & 42.233712 & 60.645323 & \nodata & \nodata & \nodata & 14.52(02) & 13.70(01) & 12.71(06) & 11.57(09) & 7.44(20) & AGN & 0.01 \\
g116 & 42.235171 & 60.803048 & 16.85(17) & 15.48(12) & 15.10(13) & 14.23(02) & 13.81(02) & 12.96(14) & 11.61(17) & \nodata & AGN & 0.01 \\
g117 & 42.273402 & 59.625261 & 15.13(05) & 14.82(07) & 14.66(09) & 14.32(02) & 14.32(02) & 14.25(08) & 13.72(13) & \nodata & AGN & 0.31 \\
g118 & 42.275718 & 60.473459 & \nodata & \nodata & \nodata & 15.04(03) & 14.13(03) & 13.09(07) & 11.91(13) & 8.74(13) & AGN & 0.01 \\
g119 & 42.301466 & 60.144911 & 15.32(06) & 14.72(10) & 14.45(09) & 14.50(02) & 14.52(02) & 14.69(20) & 13.87(20) & \nodata & AGN & 0.30 \\
g120 & 42.305054 & 59.588351 & \nodata & \nodata & \nodata & 15.70(03) & 15.16(04) & 14.26(08) & 13.49(12) & 9.11(07) & AGN & 0.09 \\
g121 & 42.307257 & 59.697057 & 15.39(05) & 14.60(06) & 14.43(08) & 14.42(02) & 14.38(02) & 14.14(12) & 13.05(12) & \nodata & AGN & 0.33 \\
g122 & 42.308391 & 59.615925 & 16.39(13) & 15.74(16) & \nodata & 15.07(03) & 14.93(03) & 14.51(12) & 13.85(14) & \nodata & AGN & 0.06 \\
g123 & 42.324468 & 60.019748 & \nodata & \nodata & \nodata & 15.28(03) & 14.98(03) & 14.33(13) & 11.71(06) & \nodata & PAH & 0.00 \\
g124 & 42.328469 & 60.182834 & \nodata & \nodata & \nodata & 15.32(02) & 14.85(04) & 14.97(19) & 12.74(09) & \nodata & PAH & 0.00 \\
g125 & 42.330419 & 60.035021 & \nodata & \nodata & \nodata & 15.32(10) & 14.94(06) & 14.35(12) & 13.22(14) & \nodata & AGN & 0.05 \\
g126 & 42.337209 & 59.689849 & \nodata & \nodata & \nodata & 15.07(02) & 14.82(04) & 14.34(11) & 12.52(09) & \nodata & PAH & 0.00 \\
g127 & 42.340698 & 60.904853 & \nodata & \nodata & \nodata & 15.64(07) & 14.81(04) & 13.77(12) & 12.32(09) & \nodata & AGN & 0.02 \\
g128 & 42.363647 & 60.563456 & \nodata & \nodata & \nodata & 14.99(02) & 13.92(02) & 13.20(09) & 11.91(13) & 8.44(17) & AGN & 0.04 \\
g129 & 42.366957 & 60.233598 & \nodata & \nodata & \nodata & 15.89(05) & 15.28(04) & 14.46(11) & 13.56(10) & \nodata & AGN & 0.04 \\
g130 & 42.392511 & 60.305948 & \nodata & \nodata & \nodata & 16.47(08) & 15.61(06) & 14.50(15) & 13.23(17) & \nodata & AGN & 0.00 \\
g131 & 42.398046 & 60.537282 & \nodata & \nodata & \nodata & 15.48(04) & 14.23(02) & 13.28(08) & 12.03(11) & \nodata & AGN & 0.04 \\
g132 & 42.398620 & 60.410258 & 14.71(04) & 14.27(06) & 14.21(07) & 14.00(01) & 13.96(02) & 13.86(09) & 12.69(10) & \nodata & PAH & 0.00 \\
g133 & 42.399398 & 60.835566 & \nodata & \nodata & \nodata & 16.35(08) & 15.35(05) & 14.44(18) & 13.79(20) & \nodata & AGN & 0.04 \\
g134 & 42.401336 & 59.476574 & \nodata & \nodata & \nodata & 15.06(02) & 14.80(04) & 14.44(18) & 13.34(13) & \nodata & AGN & 0.12 \\
g135 & 42.415541 & 60.176578 & \nodata & \nodata & \nodata & 15.86(05) & 15.52(05) & 14.78(18) & 13.68(11) & \nodata & AGN & 0.00 \\
g136 & 42.424186 & 60.259911 & \nodata & \nodata & \nodata & 15.67(03) & 14.88(03) & 13.97(09) & 12.98(07) & \nodata & AGN & 0.07 \\
g137 & 42.435021 & 60.807674 & \nodata & \nodata & \nodata & 15.52(03) & 14.01(02) & 13.25(05) & 12.37(07) & 8.12(06) & AGN & 0.06 \\
g138 & 42.440896 & 59.899957 & 15.84(07) & 15.12(08) & 14.73(10) & 14.46(01) & 14.38(02) & 14.18(09) & 13.03(13) & \nodata & AGN & 0.15 \\
g139 & 42.444426 & 60.647210 & \nodata & \nodata & \nodata & 14.50(03) & 14.18(02) & 13.28(13) & 11.88(14) & \nodata & AGN & 0.02 \\
g140 & 42.446592 & 60.568824 & \nodata & \nodata & \nodata & 14.78(03) & 14.06(02) & 13.50(10) & 12.40(13) & \nodata & AGN & 0.25 \\
g141 & 42.453758 & 60.188642 & 16.16(07) & 15.15(10) & 15.14(14) & 14.87(02) & 14.81(02) & 14.68(14) & 14.05(12) & \nodata & AGN & 0.33 \\
g142 & 42.460532 & 60.439279 & \nodata & \nodata & \nodata & 15.03(03) & 14.50(03) & 13.48(11) & 12.12(12) & \nodata & AGN & 0.02 \\
g143 & 42.460750 & 60.903031 & \nodata & \nodata & \nodata & 15.00(03) & 14.55(02) & 14.03(10) & 11.72(06) & 8.50(11) & PAH & 0.00 \\
g144 & 42.461400 & 59.456410 & \nodata & \nodata & \nodata & 15.57(03) & 14.66(03) & 13.51(06) & 12.27(05) & 8.74(08) & AGN & 0.02 \\
g145 & 42.478747 & 60.701170 & 14.58(03) & 13.43(04) & 12.90(03) & 12.34(02) & 12.16(03) & 10.99(09) & 9.26(09) & \nodata & PAH & 0.00 \\
g146 & 42.493366 & 60.392465 & \nodata & \nodata & \nodata & 17.38(17) & 16.14(08) & 14.77(12) & 13.99(14) & \nodata & AGN & 0.00 \\
g147 & 42.496340 & 60.025855 & \nodata & \nodata & \nodata & 14.57(02) & 14.40(03) & 13.49(05) & 10.70(01) & 8.07(08) & PAH & 0.00 \\
g148 & 42.512314 & 59.985275 & 14.19(03) & 13.33(04) & 13.05(03) & 12.81(01) & 12.97(01) & 12.64(05) & 11.71(05) & \nodata & PAH & 0.14 \\
g149 & 42.520215 & 60.659033 & \nodata & \nodata & \nodata & 15.21(03) & 14.85(05) & 13.91(13) & 12.39(12) & \nodata & AGN & 0.01 \\
g150 & 42.522520 & 60.238602 & 16.76(14) & 16.02(20) & 15.54(20) & 14.89(02) & 14.65(03) & 14.51(12) & 13.81(10) & \nodata & AGN & 0.58 \\
g151 & 42.522935 & 59.695176 & 15.22(05) & 14.51(06) & 14.26(07) & 14.17(01) & 14.19(02) & 14.07(12) & 12.98(18) & \nodata & PAH & 0.04 \\
g152 & 42.523580 & 60.161222 & \nodata & \nodata & \nodata & 16.12(04) & 15.53(04) & 14.86(12) & 14.01(12) & \nodata & AGN & 0.00 \\
g153 & 42.528473 & 60.352713 & \nodata & \nodata & \nodata & 15.61(06) & 14.79(05) & 14.02(09) & 12.89(06) & \nodata & AGN & 0.07 \\
g154 & 42.544542 & 60.617335 & 15.87(07) & 15.19(09) & 14.78(11) & 14.29(01) & 14.12(02) & 14.26(17) & 13.01(17) & \nodata & PAH & 0.00 \\
g155 & 42.557039 & 59.893385 & \nodata & \nodata & \nodata & 15.55(06) & 14.77(03) & 13.59(10) & 12.29(14) & 7.59(19) & AGN & 0.02 \\
g156 & 42.560692 & 60.465546 & 16.08(08) & 15.21(09) & 15.07(13) & 14.52(02) & 14.52(03) & 13.29(06) & 11.67(03) & \nodata & PAH & 0.00 \\
g157 & 42.565037 & 60.213032 & \nodata & \nodata & \nodata & 15.04(02) & 14.45(02) & 13.89(07) & 12.58(05) & \nodata & AGN & 0.15 \\
g158 & 42.565821 & 60.220892 & \nodata & \nodata & \nodata & 15.40(04) & 14.92(04) & 14.55(17) & 12.89(07) & 9.53(13) & PAH & 0.00 \\
g159 & 42.580546 & 60.236393 & \nodata & \nodata & \nodata & 16.04(04) & 15.17(04) & 14.14(07) & 13.47(09) & \nodata & AGN & 0.13 \\
g160 & 42.583700 & 60.300753 & 16.18(09) & 15.26(10) & 15.10(14) & 14.10(01) & 13.65(01) & 13.20(04) & 11.97(04) & 9.41(38) & AGN & 0.26 \\
g161 & 42.586206 & 59.437430 & 15.52(06) & 14.77(07) & 14.70(09) & 14.54(01) & 14.46(02) & 14.47(12) & 13.88(09) & \nodata & AGN & 0.40 \\
g162 & 42.587418 & 60.297174 & 16.43(10) & 15.52(11) & 14.84(11) & 14.54(02) & 14.18(02) & 13.86(08) & 12.85(06) & \nodata & AGN & 0.39 \\
g163 & 42.589327 & 60.450975 & 16.55(13) & 15.60(14) & 15.35(17) & 14.90(02) & 14.78(03) & 14.48(12) & 13.43(09) & \nodata & AGN & 0.44 \\
g164 & 42.594924 & 60.884663 & \nodata & \nodata & \nodata & 14.72(04) & 14.58(03) & 13.57(16) & 10.93(08) & 8.00(20) & PAH & 0.00 \\
g165 & 42.599874 & 60.459478 & \nodata & \nodata & \nodata & 15.15(02) & 14.34(02) & 13.51(05) & 12.26(03) & \nodata & AGN & 0.09 \\
g166 & 42.615653 & 60.439974 & 16.80(15) & \nodata & 15.49(19) & 15.11(02) & 14.80(03) & 14.47(11) & 13.68(11) & \nodata & AGN & 0.56 \\
g167 & 42.620283 & 60.652211 & 16.94(17) & 15.64(13) & 14.98(12) & 14.40(02) & 14.16(02) & 13.42(09) & 12.01(10) & \nodata & AGN & 0.05 \\
g168 & 42.622004 & 60.465652 & 15.50(05) & 14.85(06) & 14.60(08) & 14.50(01) & 14.43(02) & 14.43(11) & 13.41(11) & \nodata & PAH & 0.46 \\
g169 & 42.630672 & 60.585930 & \nodata & \nodata & \nodata & 15.38(03) & 14.72(03) & 14.15(11) & 13.60(16) & \nodata & AGN & 0.32 \\
g170 & 42.631048 & 60.593540 & 15.49(05) & 14.66(07) & 14.40(08) & 13.77(01) & 13.68(02) & 13.38(11) & 12.12(18) & 7.95(07) & PAH & 0.00 \\
g171 & 42.631494 & 59.868286 & \nodata & \nodata & \nodata & 15.00(03) & 14.05(02) & 13.25(07) & 11.66(07) & 7.20(07) & AGN & 0.01 \\
g172 & 42.633248 & 60.426204 & 15.44(05) & 14.68(05) & 14.40(07) & 14.23(01) & 14.18(02) & 14.05(07) & 13.59(09) & \nodata & AGN & 0.80 \\
g173 & 42.637543 & 60.257163 & \nodata & \nodata & \nodata & 16.25(05) & 15.46(04) & 14.38(10) & 13.77(13) & \nodata & AGN & 0.07 \\
g174 & 42.641719 & 59.555931 & 15.71(07) & 15.32(13) & 14.73(11) & 14.83(02) & 14.77(03) & 14.81(16) & 13.96(17) & \nodata & AGN & 0.24 \\
g175 & 42.652709 & 60.181903 & \nodata & \nodata & \nodata & 15.89(04) & 15.18(04) & 14.16(09) & 13.77(13) & \nodata & AGN & 0.17 \\
g176 & 42.658746 & 59.921043 & \nodata & \nodata & \nodata & 15.64(05) & 14.82(04) & 13.18(06) & 10.92(02) & 5.86(04) & PAH & 0.00 \\
g177 & 42.665237 & 60.391484 & 16.63(16) & 15.51(14) & 15.41(17) & 14.82(02) & 14.58(03) & 14.15(09) & 13.41(07) & \nodata & AGN & 0.71 \\
g178 & 42.668848 & 60.173564 & 15.24(07) & 14.64(06) & 14.34(06) & 14.20(01) & 14.21(02) & 14.04(09) & 13.65(14) & \nodata & AGN & 0.36 \\
g179 & 42.670310 & 60.407272 & 16.81(17) & 15.82(18) & 15.34(17) & 14.63(02) & 14.46(02) & 14.27(12) & 13.78(11) & \nodata & AGN & 0.79 \\
g180 & 42.671798 & 60.424345 & 16.61(12) & 15.55(13) & 15.09(14) & 14.43(01) & 14.01(02) & 13.56(05) & 12.60(05) & \nodata & AGN & 0.71 \\
g181 & 42.678738 & 60.161140 & \nodata & \nodata & \nodata & 15.85(04) & 15.50(04) & 14.88(16) & 13.05(06) & \nodata & PAH & 0.00 \\
g182 & 42.680343 & 59.611217 & \nodata & \nodata & \nodata & 15.26(05) & 14.52(03) & 13.35(07) & 11.94(04) & 8.26(07) & AGN & 0.01 \\
g183 & 42.681662 & 60.164090 & \nodata & \nodata & \nodata & 15.02(04) & 14.62(04) & 13.90(10) & 12.38(05) & 8.84(13) & AGN & 0.06 \\
g184 & 42.681947 & 60.450036 & 16.29(10) & 15.18(09) & 14.85(12) & 14.50(02) & 14.43(02) & 14.46(11) & 13.62(11) & \nodata & AGN & 0.74 \\
g185 & 42.682937 & 60.527487 & \nodata & \nodata & 15.11(16) & 14.20(03) & 13.87(03) & 13.29(09) & 10.66(06) & 7.53(07) & PAH & 0.00 \\
g186 & 42.683127 & 60.438306 & 15.80(08) & 14.99(07) & 14.72(10) & 14.49(01) & 14.26(02) & 13.89(07) & 12.87(05) & \nodata & AGN & 0.70 \\
g187 & 42.685047 & 60.410765 & \nodata & \nodata & \nodata & 15.01(03) & 14.68(02) & 14.42(11) & 13.56(09) & \nodata & AGN & 0.71 \\
g188 & 42.693030 & 60.397422 & 16.61(14) & 16.00(19) & \nodata & 14.63(03) & 14.39(03) & 14.24(09) & 13.70(12) & \nodata & AGN & 0.80 \\
g189 & 42.694360 & 59.628806 & 15.32(06) & 14.55(06) & 14.38(07) & 14.19(01) & 14.15(02) & 14.02(10) & 13.62(14) & \nodata & AGN & 0.18 \\
g190 & 42.695597 & 60.092080 & \nodata & \nodata & \nodata & 15.63(05) & 15.18(05) & 14.55(17) & 13.85(14) & 9.56(12) & AGN & 0.14 \\
g191 & 42.695856 & 60.393617 & \nodata & \nodata & \nodata & 15.21(03) & 14.18(02) & 13.45(07) & 12.39(05) & 11.10(87) & AGN & 0.19 \\
g192 & 42.696463 & 60.339905 & 16.35(09) & 15.84(16) & 15.08(13) & 14.40(02) & 14.11(02) & 13.71(07) & 12.74(06) & \nodata & AGN & 0.68 \\
g193 & 42.698204 & 60.637997 & \nodata & \nodata & \nodata & 15.47(04) & 14.97(04) & 14.65(16) & 13.38(13) & 9.17(12) & AGN & 0.23 \\
g194 & 42.698910 & 60.355059 & 16.38(12) & 15.55(12) & 15.40(18) & 14.88(02) & 14.73(04) & 14.36(11) & 13.69(11) & \nodata & AGN & 0.68 \\
g195 & 42.701765 & 60.386916 & \nodata & \nodata & \nodata & 15.36(04) & 15.06(04) & 14.39(13) & 13.61(12) & \nodata & AGN & 0.31 \\
g196 & 42.703761 & 60.396290 & 16.41(12) & 15.33(10) & 14.89(11) & 14.75(02) & 14.66(03) & 14.31(13) & 13.42(17) & \nodata & AGN & 0.71 \\
g197 & 42.708336 & 60.969102 & 13.38(03) & 12.85(03) & 12.72(03) & 12.69(01) & 12.67(01) & 12.05(09) & 10.74(12) & \nodata & PAH & 0.00 \\
g198 & 42.708710 & 60.095839 & 15.27(06) & 14.67(06) & 14.48(08) & 14.46(01) & 14.52(02) & 14.55(12) & 13.98(14) & \nodata & AGN & 0.34 \\
g199 & 42.709176 & 60.505110 & 16.51(10) & 15.67(14) & 15.45(18) & 15.03(02) & 14.71(03) & 14.20(10) & 13.37(12) & \nodata & AGN & 0.53 \\
g200 & 42.718283 & 60.404298 & \nodata & \nodata & \nodata & 14.50(02) & 14.20(02) & 14.07(11) & 13.69(18) & \nodata & AGN & 0.80 \\
g201 & 42.718655 & 60.452461 & 16.26(11) & 15.12(09) & 15.06(13) & 14.57(01) & 14.41(02) & 14.43(10) & 13.40(12) & \nodata & PAH & 0.43 \\
g202 & 42.719454 & 60.371205 & 16.59(13) & 15.69(13) & 14.88(11) & 14.17(01) & 13.64(01) & 12.97(03) & 11.99(04) & 8.85(08) & AGN & 0.48 \\
g203 & 42.719620 & 60.291189 & \nodata & \nodata & \nodata & 16.14(05) & 15.47(06) & 14.72(15) & 13.83(14) & \nodata & AGN & 0.07 \\
g204 & 42.719901 & 60.460649 & \nodata & \nodata & \nodata & 15.01(04) & 14.83(06) & 14.33(12) & 12.28(04) & \nodata & PAH & 0.00 \\
g205 & 42.722333 & 60.429956 & \nodata & \nodata & \nodata & 14.97(02) & 14.57(03) & 14.39(12) & 13.98(14) & \nodata & AGN & 0.76 \\
g206 & 42.730185 & 59.852514 & \nodata & \nodata & \nodata & 15.13(03) & 14.38(02) & 13.86(08) & 12.69(09) & 9.17(08) & AGN & 0.06 \\
g207 & 42.731394 & 59.808664 & \nodata & \nodata & \nodata & 14.84(03) & 14.58(03) & 13.84(08) & 11.33(04) & 7.60(06) & PAH & 0.00 \\
g208 & 42.733916 & 60.445304 & 15.20(07) & 14.22(07) & 13.68(06) & 13.11(01) & 12.93(01) & 12.56(03) & 11.10(02) & 8.31(07) & PAH & 0.00 \\
g209 & 42.734817 & 60.372009 & 16.14(09) & 15.28(09) & 15.01(12) & 14.62(02) & 14.50(03) & 14.35(11) & 13.84(19) & 9.29(18) & AGN & 0.79 \\
g210 & 42.737571 & 60.565918 & \nodata & \nodata & \nodata & 14.88(04) & 14.43(03) & 13.75(16) & 12.43(18) & \nodata & AGN & 0.09 \\
g211 & 42.738649 & 60.512452 & 17.06(19) & 16.06(18) & 15.32(16) & 14.88(02) & 14.65(02) & 14.68(16) & 13.78(11) & \nodata & AGN & 0.58 \\
g212 & 42.744411 & 60.443287 & 15.30(04) & 14.87(07) & 14.67(09) & 14.68(02) & 14.64(03) & 14.50(12) & 13.65(12) & \nodata & AGN & 0.73 \\
g213 & 42.746705 & 60.386170 & \nodata & \nodata & \nodata & 15.14(02) & 14.66(03) & 14.42(11) & 13.61(11) & \nodata & AGN & 0.71 \\
g214 & 42.748794 & 60.403900 & \nodata & 15.79(17) & 15.18(15) & 14.40(03) & 14.04(03) & 13.38(06) & 12.56(06) & 8.99(12) & AGN & 0.71 \\
g215 & 42.751389 & 60.371768 & \nodata & \nodata & \nodata & 15.25(02) & 14.88(03) & 14.30(11) & 13.89(12) & \nodata & AGN & 0.60 \\
g216 & 42.751624 & 60.583698 & \nodata & \nodata & \nodata & 14.87(04) & 14.28(03) & 13.73(12) & 12.42(14) & 8.59(10) & AGN & 0.15 \\
g217 & 42.761679 & 60.304945 & \nodata & \nodata & \nodata & 14.92(02) & 14.55(02) & 14.21(07) & 13.41(07) & \nodata & AGN & 0.68 \\
g218 & 42.761839 & 60.453997 & \nodata & \nodata & \nodata & 15.22(02) & 15.02(03) & 14.83(13) & 14.05(18) & \nodata & AGN & 0.34 \\
g219 & 42.762413 & 60.382483 & \nodata & \nodata & \nodata & 15.05(02) & 14.78(02) & 14.62(12) & 14.00(13) & \nodata & AGN & 0.60 \\
g220 & 42.767914 & 60.769898 & \nodata & \nodata & \nodata & 14.99(04) & 14.63(03) & 13.97(10) & 12.73(17) & \nodata & AGN & 0.02 \\
g221 & 42.773815 & 60.244989 & \nodata & \nodata & \nodata & 14.84(02) & 14.78(03) & 14.54(10) & 13.87(15) & \nodata & AGN & 0.48 \\
g222 & 42.782568 & 60.389706 & 17.03(20) & 16.05(20) & 15.68(23) & 14.87(03) & 14.54(03) & 14.44(11) & 13.65(14) & \nodata & AGN & 0.73 \\
g223 & 42.782612 & 60.337095 & 15.27(10) & 14.44(07) & 14.34(07) & 14.17(01) & 14.19(03) & 14.26(14) & 13.20(11) & \nodata & PAH & 0.73 \\
g224 & 42.783786 & 60.346389 & \nodata & \nodata & \nodata & 15.53(04) & 15.09(03) & 14.76(19) & 13.73(14) & \nodata & AGN & 0.31 \\
g225 & 42.784160 & 60.433458 & 16.06(11) & 15.33(13) & 14.98(14) & 14.43(04) & 14.27(04) & 14.27(15) & 13.66(11) & \nodata & AGN & 0.79 \\
g226 & 42.784684 & 60.363801 & \nodata & \nodata & \nodata & 15.32(03) & 14.97(03) & 14.47(09) & 13.78(15) & 9.53(12) & AGN & 0.59 \\
g227 & 42.786195 & 60.448410 & \nodata & \nodata & \nodata & 15.50(04) & 14.90(03) & 14.30(11) & 13.64(10) & \nodata & AGN & 0.55 \\
g228 & 42.786255 & 59.262206 & \nodata & \nodata & \nodata & 15.16(05) & 14.43(04) & 13.60(11) & 12.47(06) & \nodata & AGN & 0.10 \\
g229 & 42.787452 & 60.315115 & 16.79(16) & 15.43(13) & 15.07(13) & 14.56(02) & 14.21(02) & 13.90(08) & 13.55(09) & \nodata & AGN & 0.80 \\
g230 & 42.790691 & 60.363048 & \nodata & \nodata & \nodata & 15.13(03) & 14.77(03) & 14.74(15) & 13.44(13) & \nodata & PAH & 0.00 \\
g231 & 42.793994 & 60.436461 & \nodata & \nodata & \nodata & 14.76(07) & 14.31(06) & 13.85(09) & 13.04(09) & \nodata & AGN & 0.70 \\
g232 & 42.794280 & 60.238273 & \nodata & \nodata & \nodata & 15.27(02) & 15.38(04) & 14.79(20) & 13.09(09) & \nodata & PAH & 0.00 \\
g233 & 42.795084 & 60.371918 & 16.72(16) & 15.71(14) & 15.21(15) & 14.81(02) & 14.53(04) & 13.99(09) & 13.28(14) & \nodata & AGN & 0.67 \\
g234 & 42.796658 & 60.282662 & 15.83(07) & 15.20(09) & 15.23(14) & 14.81(03) & 14.90(03) & 14.81(14) & 13.58(11) & \nodata & PAH & 0.46 \\
g235 & 42.798653 & 60.600800 & \nodata & \nodata & \nodata & 15.44(03) & 15.17(04) & 14.68(18) & 13.92(14) & \nodata & AGN & 0.32 \\
g236 & 42.798997 & 60.343611 & 16.45(11) & 15.70(14) & 15.53(20) & 14.93(02) & 14.73(02) & 14.52(11) & 13.64(13) & \nodata & AGN & 0.71 \\
g237 & 42.799341 & 60.408005 & 16.36(14) & 15.36(14) & 15.08(17) & 14.69(06) & 14.46(06) & 14.41(13) & 13.55(14) & \nodata & AGN & 0.77 \\
g238 & 42.799722 & 60.442044 & \nodata & \nodata & \nodata & 15.14(03) & 14.65(03) & 14.06(10) & 12.80(06) & 9.21(09) & AGN & 0.18 \\
g239 & 42.799944 & 60.521700 & 16.63(12) & 15.42(11) & 14.97(14) & 14.82(02) & 14.52(02) & 14.18(09) & 12.96(06) & \nodata & AGN & 0.48 \\
g240 & 42.803535 & 60.657759 & \nodata & \nodata & \nodata & 14.51(02) & 14.10(02) & 13.53(09) & 12.71(12) & \nodata & AGN & 0.56 \\
g241 & 42.807869 & 59.854407 & \nodata & \nodata & \nodata & 15.45(04) & 14.93(03) & 13.91(07) & 13.09(10) & 10.26(23) & AGN & 0.03 \\
g242 & 42.808976 & 60.473082 & 16.05(09) & 15.22(12) & 14.92(12) & 14.42(02) & 14.28(03) & 14.07(08) & 13.67(11) & \nodata & AGN & 0.79 \\
g243 & 42.809427 & 60.248827 & \nodata & \nodata & \nodata & 15.13(02) & 14.87(03) & 14.53(16) & 13.92(14) & \nodata & AGN & 0.58 \\
g244 & 42.810962 & 60.427895 & \nodata & \nodata & \nodata & 14.69(04) & 14.36(04) & 14.24(10) & 13.69(12) & \nodata & AGN & 0.79 \\
g245 & 42.811235 & 60.504765 & \nodata & \nodata & \nodata & 14.85(03) & 14.25(02) & 13.77(07) & 12.80(07) & 9.64(19) & AGN & 0.67 \\
g246 & 42.812653 & 60.424301 & 16.29(11) & 15.36(12) & \nodata & 14.25(02) & 13.87(02) & 13.69(08) & 12.45(05) & 7.67(09) & PAH & 0.00 \\
g247 & 42.813604 & 60.628054 & 16.45(11) & 15.33(10) & 15.11(14) & 14.69(02) & 14.23(02) & 13.80(09) & 12.53(15) & \nodata & AGN & 0.51 \\
g248 & 42.815396 & 59.773858 & \nodata & \nodata & \nodata & 15.10(03) & 14.58(03) & 14.31(08) & 11.99(04) & 9.10(10) & PAH & 0.00 \\
g249 & 42.816680 & 60.332858 & \nodata & \nodata & \nodata & 15.18(03) & 14.81(03) & 14.67(16) & 13.46(12) & \nodata & PAH & 0.00 \\
g250 & 42.816976 & 60.462588 & \nodata & \nodata & \nodata & 15.78(04) & 15.17(04) & 14.27(10) & 13.28(10) & 8.97(10) & AGN & 0.08 \\
g251 & 42.819303 & 60.313153 & 16.60(12) & \nodata & \nodata & 14.70(02) & 14.41(02) & 14.19(09) & 13.61(10) & \nodata & AGN & 0.77 \\
g252 & 42.819899 & 60.302601 & \nodata & \nodata & \nodata & 15.20(02) & 14.91(03) & 14.74(12) & 13.74(08) & \nodata & AGN & 0.59 \\
g253 & 42.820086 & 60.365021 & \nodata & \nodata & \nodata & 14.53(03) & 13.89(03) & 13.22(04) & 12.41(05) & 8.78(08) & AGN & 0.62 \\
g254 & 42.820294 & 60.659434 & 15.67(05) & 15.13(09) & 14.78(10) & 14.51(02) & 14.42(03) & 14.40(16) & 13.38(16) & \nodata & PAH & 0.00 \\
g255 & 42.820549 & 60.291921 & 16.54(12) & 15.88(17) & 15.07(14) & 14.72(01) & 14.46(02) & 14.14(09) & 13.70(13) & \nodata & AGN & 0.77 \\
g256 & 42.823705 & 60.335843 & \nodata & \nodata & \nodata & 14.43(01) & 13.86(01) & 13.19(05) & 12.31(06) & \nodata & AGN & 0.47 \\
g257 & 42.824936 & 60.605300 & \nodata & \nodata & \nodata & 14.55(02) & 14.33(02) & 14.12(11) & 13.67(15) & \nodata & AGN & 0.76 \\
g258 & 42.828306 & 59.573948 & 16.53(11) & 16.13(20) & 15.37(16) & 15.39(03) & 15.09(03) & 14.62(10) & 13.75(10) & 9.96(16) & AGN & 0.14 \\
g259 & 42.828768 & 60.002740 & \nodata & \nodata & \nodata & 15.22(02) & 14.47(02) & 13.59(06) & 13.02(06) & \nodata & AGN & 0.28 \\
g260 & 42.829279 & 60.539306 & \nodata & \nodata & \nodata & 14.65(03) & 14.22(03) & 14.13(07) & 13.68(09) & \nodata & AGN & 0.80 \\
g261 & 42.832882 & 60.737232 & \nodata & \nodata & \nodata & 15.08(06) & 14.46(03) & 13.32(12) & 11.89(15) & \nodata & AGN & 0.02 \\
g262 & 42.834369 & 60.235945 & 15.46(04) & 14.90(07) & 14.72(09) & 14.62(02) & 14.64(03) & 14.92(20) & 13.87(12) & \nodata & PAH & 0.61 \\
g263 & 42.834676 & 60.532505 & \nodata & \nodata & \nodata & 14.87(02) & 14.37(02) & 14.33(11) & 13.55(09) & \nodata & AGN & 0.77 \\
g264 & 42.834979 & 60.286811 & \nodata & \nodata & \nodata & 15.59(05) & 15.13(04) & 14.81(17) & 12.88(06) & \nodata & PAH & 0.00 \\
g265 & 42.835818 & 60.364944 & 16.52(11) & 15.91(19) & 15.63(22) & 14.62(02) & 14.42(03) & 14.11(10) & 13.77(10) & \nodata & AGN & 0.79 \\
g266 & 42.839931 & 60.389812 & 16.93(17) & 15.95(19) & 15.41(17) & 14.84(04) & 14.46(04) & 14.21(13) & 13.57(14) & \nodata & AGN & 0.77 \\
g267 & 42.841135 & 60.575526 & \nodata & \nodata & \nodata & 15.04(02) & 14.48(03) & 14.32(10) & 13.68(18) & \nodata & AGN & 0.74 \\
g268 & 42.841237 & 60.482157 & 17.13(19) & 15.68(13) & 15.48(18) & 14.66(02) & 14.35(03) & 14.06(08) & 13.75(16) & \nodata & AGN & 0.79 \\
g269 & 42.846000 & 60.565328 & 15.37(07) & 14.39(06) & 13.79(05) & 13.53(01) & 13.28(01) & 13.06(04) & 11.74(03) & 7.96(07) & PAH & 0.00 \\
g270 & 42.847173 & 60.359486 & \nodata & \nodata & \nodata & 15.04(02) & 14.62(03) & 14.18(07) & 13.67(09) & \nodata & AGN & 0.73 \\
g271 & 42.847717 & 60.372734 & 16.48(11) & 15.62(12) & 15.15(13) & 14.46(02) & 14.19(02) & 13.85(06) & 13.55(10) & \nodata & AGN & 0.80 \\
g272 & 42.848906 & 60.550098 & 16.41(10) & 15.45(12) & 15.05(13) & 14.92(02) & 14.88(03) & 14.60(13) & 13.54(15) & 9.66(21) & AGN & 0.55 \\
g273 & 42.850245 & 60.441959 & \nodata & \nodata & \nodata & 14.90(02) & 14.52(03) & 14.13(09) & 13.28(07) & \nodata & AGN & 0.71 \\
g274 & 42.850545 & 60.279654 & 16.16(09) & 15.15(07) & 14.95(12) & 14.19(01) & 13.79(01) & 13.26(04) & 12.33(05) & \nodata & AGN & 0.62 \\
g275 & 42.853187 & 60.270066 & 16.61(13) & 15.84(15) & 15.37(15) & 14.99(02) & 14.71(03) & 14.26(09) & 13.66(17) & \nodata & AGN & 0.71 \\
g276 & 42.856504 & 59.508384 & \nodata & \nodata & \nodata & 16.73(11) & 15.41(07) & 14.45(14) & 13.48(10) & 9.44(14) & AGN & 0.01 \\
g277 & 42.857062 & 60.449067 & \nodata & \nodata & \nodata & 16.25(11) & 15.28(07) & 14.56(15) & 13.96(15) & \nodata & AGN & 0.12 \\
g278 & 42.857251 & 60.092718 & \nodata & \nodata & \nodata & 15.00(03) & 14.39(03) & 13.90(08) & 12.78(07) & \nodata & AGN & 0.29 \\
g279 & 42.859160 & 60.550713 & \nodata & \nodata & \nodata & 15.52(04) & 15.10(04) & 14.90(18) & 14.16(16) & \nodata & AGN & 0.34 \\
g280 & 42.861341 & 61.155664 & 14.94(04) & 14.22(05) & 13.99(05) & 13.86(01) & 13.84(01) & 14.04(11) & 12.77(12) & \nodata & PAH & 0.36 \\
g281 & 42.862808 & 60.471236 & \nodata & \nodata & \nodata & 14.99(03) & 14.54(03) & 14.22(17) & 13.29(13) & 9.00(09) & AGN & 0.67 \\
g282 & 42.864847 & 61.034564 & \nodata & \nodata & \nodata & 14.97(03) & 14.11(02) & 13.42(09) & 12.13(12) & 8.91(21) & AGN & 0.10 \\
g283 & 42.865924 & 60.004247 & 16.00(07) & 15.60(12) & 15.03(11) & 14.83(02) & 14.82(03) & 14.55(12) & 12.98(09) & \nodata & PAH & 0.00 \\
g284 & 42.866690 & 60.545007 & \nodata & \nodata & \nodata & 15.02(03) & 14.08(02) & 13.45(06) & 12.52(05) & \nodata & AGN & 0.53 \\
g285 & 42.866959 & 59.925751 & \nodata & \nodata & \nodata & 15.12(04) & 14.83(04) & 14.14(14) & 11.43(06) & 8.16(08) & PAH & 0.00 \\
g286 & 42.867927 & 60.439836 & \nodata & \nodata & \nodata & 14.59(02) & 14.30(02) & 13.92(08) & 13.71(10) & \nodata & AGN & 0.76 \\
g287 & 42.869495 & 60.622961 & 16.68(12) & 15.46(10) & 14.98(11) & 14.51(02) & 14.08(02) & 13.60(05) & 12.44(04) & 9.13(09) & AGN & 0.51 \\
g288 & 42.869649 & 60.310407 & 16.50(11) & 15.19(09) & 15.14(15) & 14.70(02) & 14.38(02) & 14.17(08) & 13.62(08) & \nodata & AGN & 0.77 \\
g289 & 42.871661 & 60.376730 & 15.67(07) & 14.76(06) & 14.44(07) & 14.34(01) & 14.33(02) & 14.31(11) & 13.78(12) & \nodata & AGN & 0.79 \\
g290 & 42.872909 & 60.176272 & 16.71(15) & 16.21(21) & 15.49(18) & 15.03(02) & 14.69(03) & 14.00(08) & 12.76(06) & 8.55(07) & AGN & 0.17 \\
g291 & 42.880059 & 60.486381 & \nodata & \nodata & \nodata & 14.58(02) & 13.67(01) & 11.72(02) & 9.71(01) & 6.10(04) & PAH & 0.65 \\
g292 & 42.880770 & 60.493494 & \nodata & \nodata & \nodata & 15.45(05) & 14.83(05) & 14.33(12) & 13.68(17) & \nodata & AGN & 0.56 \\
g293 & 42.882481 & 60.308942 & \nodata & \nodata & \nodata & 16.91(08) & 15.82(06) & 14.63(11) & 13.26(09) & \nodata & AGN & 0.00 \\
g294 & 42.882555 & 60.211803 & \nodata & \nodata & \nodata & 14.38(02) & 13.78(01) & 13.14(04) & 12.18(03) & 8.93(09) & AGN & 0.45 \\
g295 & 42.883183 & 60.525877 & 16.80(15) & 15.91(17) & \nodata & 15.17(03) & 14.90(03) & 14.45(11) & 13.73(15) & \nodata & AGN & 0.59 \\
g296 & 42.885055 & 60.192069 & 16.74(15) & \nodata & \nodata & 15.51(03) & 15.34(04) & 14.96(19) & 14.10(20) & \nodata & AGN & 0.12 \\
g297 & 42.887701 & 60.370917 & \nodata & \nodata & \nodata & 15.21(03) & 14.75(03) & 14.33(10) & 13.53(11) & \nodata & AGN & 0.71 \\
g298 & 42.888717 & 60.284084 & \nodata & \nodata & \nodata & 15.79(04) & 15.37(04) & 15.11(16) & 13.96(12) & \nodata & AGN & 0.12 \\
g299 & 42.890790 & 60.320432 & \nodata & \nodata & \nodata & 15.40(03) & 14.98(03) & 14.71(12) & 13.99(12) & \nodata & AGN & 0.60 \\
g300 & 42.892233 & 60.256509 & \nodata & \nodata & \nodata & 15.15(03) & 14.11(02) & 13.13(05) & 11.96(04) & 8.54(08) & AGN & 0.11 \\
g301 & 42.892703 & 60.596318 & 14.86(04) & 14.05(05) & 13.66(04) & 13.10(01) & 12.81(01) & 12.57(03) & 11.27(03) & 7.89(07) & PAH & 0.00 \\
g302 & 42.893037 & 60.287214 & 16.52(14) & 15.95(17) & 15.05(13) & 14.25(01) & 13.81(01) & 13.31(05) & 12.35(04) & 9.10(11) & AGN & 0.62 \\
g303 & 42.898156 & 60.406540 & 16.11(12) & 15.27(10) & 14.93(14) & 14.58(02) & 14.57(03) & 14.67(12) & 13.88(13) & \nodata & AGN & 0.76 \\
g304 & 42.898443 & 60.591676 & \nodata & \nodata & \nodata & 15.09(03) & 14.51(03) & 13.99(08) & 13.21(07) & \nodata & AGN & 0.64 \\
g305 & 42.898734 & 60.646719 & 16.54(12) & 15.69(14) & 15.33(16) & 14.78(02) & 14.37(02) & 13.54(06) & 12.37(07) & \nodata & AGN & 0.15 \\
g306 & 42.900002 & 60.265977 & 14.16(03) & 13.66(04) & 13.29(04) & 12.34(01) & 12.04(01) & 11.22(01) & 9.43(01) & 4.84(06) & PAH & 0.00 \\
g307 & 42.900999 & 60.526897 & \nodata & \nodata & \nodata & 15.12(03) & 15.02(04) & 14.51(15) & 14.03(12) & \nodata & AGN & 0.32 \\
g308 & 42.902220 & 60.281553 & 16.15(11) & 15.56(14) & 15.01(14) & 14.54(01) & 14.33(02) & 14.32(10) & 13.65(10) & 9.45(17) & AGN & 0.79 \\
g309 & 42.903084 & 60.324989 & \nodata & \nodata & \nodata & 15.34(03) & 15.03(04) & 14.94(16) & 13.43(10) & 8.69(18) & PAH & 0.00 \\
g310 & 42.903778 & 60.345462 & \nodata & \nodata & \nodata & 15.79(04) & 15.24(05) & 14.37(17) & 13.09(07) & 8.51(11) & AGN & 0.05 \\
g311 & 42.909342 & 60.394227 & 16.77(19) & 15.87(20) & 14.91(13) & 14.40(02) & 14.22(02) & 13.77(08) & 11.59(03) & 8.86(07) & PAH & 0.00 \\
g312 & 42.909382 & 60.115095 & 16.20(11) & 15.09(10) & 14.64(11) & 14.13(01) & 13.60(01) & 13.02(03) & 11.73(04) & 8.04(05) & AGN & 0.17 \\
g313 & 42.910057 & 60.320476 & 16.47(12) & 15.75(14) & \nodata & 14.66(02) & 14.29(02) & 13.91(07) & 13.56(09) & \nodata & AGN & 0.79 \\
g314 & 42.910982 & 60.228847 & 15.88(08) & 15.50(13) & 14.97(12) & 14.90(02) & 14.84(02) & 14.71(13) & 14.14(16) & \nodata & AGN & 0.60 \\
g315 & 42.916935 & 60.393235 & 16.70(14) & 15.51(12) & 14.92(12) & 14.35(02) & 13.86(01) & 13.44(05) & 12.26(04) & 8.66(10) & AGN & 0.47 \\
g316 & 42.918602 & 60.561065 & 16.51(13) & 15.39(12) & 15.08(14) & 14.49(01) & 13.99(02) & 13.36(06) & 12.22(04) & 10.49(92) & AGN & 0.16 \\
g317 & 42.920344 & 60.144396 & 16.39(12) & 15.71(13) & 15.50(19) & 14.92(03) & 14.63(03) & 14.49(14) & 14.12(18) & \nodata & AGN & 0.76 \\
g318 & 42.920930 & 60.168897 & 16.69(16) & 16.11(19) & 15.06(14) & 14.82(02) & 14.44(02) & 14.29(08) & 13.18(06) & \nodata & AGN & 0.70 \\
g319 & 42.922940 & 60.384823 & \nodata & \nodata & \nodata & 15.56(04) & 15.23(04) & 14.69(12) & 14.10(12) & \nodata & AGN & 0.33 \\
g320 & 42.923996 & 60.517563 & 15.51(06) & 14.92(08) & 14.99(13) & 14.52(02) & 14.65(03) & 14.38(13) & 13.99(12) & \nodata & AGN & 0.72 \\
g321 & 42.924641 & 60.333791 & 16.64(14) & 15.84(16) & 15.35(19) & 14.80(02) & 14.21(02) & 13.53(05) & 12.31(04) & 8.66(06) & AGN & 0.19 \\
g322 & 42.926290 & 60.539929 & \nodata & \nodata & \nodata & 16.13(06) & 16.02(11) & 14.47(14) & 13.00(09) & \nodata & AGN & 0.00 \\
g323 & 42.927276 & 60.185024 & \nodata & \nodata & \nodata & 15.67(03) & 15.20(03) & 14.55(12) & 14.07(13) & \nodata & AGN & 0.33 \\
g324 & 42.930223 & 60.369450 & \nodata & \nodata & \nodata & 15.10(02) & 14.85(03) & 14.59(11) & 14.21(19) & \nodata & AGN & 0.62 \\
g325 & 42.931691 & 60.300089 & \nodata & \nodata & \nodata & 15.18(02) & 14.59(02) & 14.03(07) & 13.29(07) & \nodata & AGN & 0.67 \\
g326 & 42.932032 & 60.554934 & 16.99(18) & 15.73(15) & 15.33(17) & 14.86(02) & 14.61(03) & 14.47(13) & 13.57(09) & \nodata & AGN & 0.68 \\
g327 & 42.933044 & 59.717744 & \nodata & \nodata & \nodata & 14.52(02) & 14.42(03) & 13.24(05) & 11.53(02) & 6.76(03) & PAH & 0.00 \\
g328 & 42.934004 & 60.178604 & \nodata & \nodata & \nodata & 15.60(03) & 15.10(03) & 14.44(13) & 13.83(10) & \nodata & AGN & 0.31 \\
g329 & 42.934664 & 60.430833 & \nodata & 14.59(07) & \nodata & 14.27(01) & 14.23(02) & 14.30(11) & 13.62(11) & \nodata & AGN & 0.77 \\
g330 & 42.935469 & 60.429611 & \nodata & 15.66(14) & \nodata & 14.92(02) & 14.58(03) & 14.48(14) & 13.77(13) & \nodata & AGN & 0.70 \\
g331 & 42.936354 & 60.129457 & \nodata & \nodata & \nodata & 15.31(02) & 15.04(03) & 14.69(14) & 14.05(15) & \nodata & AGN & 0.34 \\
g332 & 42.936384 & 59.542136 & 16.81(19) & 15.47(12) & 14.57(09) & 13.96(01) & 13.34(01) & 12.46(03) & 10.46(01) & 6.66(04) & PAH & 0.00 \\
g333 & 42.937102 & 60.182596 & \nodata & \nodata & \nodata & 15.51(03) & 14.96(03) & 14.42(09) & 13.19(07) & \nodata & AGN & 0.15 \\
g334 & 42.938057 & 60.062811 & \nodata & \nodata & \nodata & 16.53(06) & 15.22(04) & 14.08(07) & 12.66(06) & 8.90(07) & AGN & 0.01 \\
g335 & 42.938892 & 60.274122 & \nodata & \nodata & \nodata & 15.09(07) & 14.87(05) & 14.64(20) & 13.44(09) & \nodata & AGN & 0.55 \\
g336 & 42.941411 & 60.177876 & \nodata & \nodata & \nodata & 15.26(03) & 14.83(03) & 14.35(12) & 13.59(11) & \nodata & AGN & 0.59 \\
g337 & 42.944063 & 60.415313 & \nodata & \nodata & \nodata & 15.93(04) & 14.89(03) & 13.65(05) & 12.33(04) & 8.86(07) & AGN & 0.03 \\
g338 & 42.948082 & 60.134235 & \nodata & \nodata & \nodata & 15.20(03) & 14.67(04) & 14.03(10) & 12.78(06) & \nodata & AGN & 0.18 \\
g339 & 42.950791 & 59.674738 & \nodata & \nodata & \nodata & 15.87(05) & 15.14(04) & 14.17(12) & 13.28(09) & 8.95(08) & AGN & 0.01 \\
g340 & 42.954610 & 60.290077 & \nodata & \nodata & \nodata & 15.26(02) & 14.27(02) & 13.39(04) & 12.13(04) & 8.98(10) & AGN & 0.10 \\
g341 & 42.955594 & 60.350308 & 16.74(17) & 15.59(12) & 15.40(19) & 14.97(02) & 14.65(03) & 14.24(08) & 13.32(08) & \nodata & AGN & 0.64 \\
g342 & 42.957794 & 60.170558 & \nodata & \nodata & \nodata & 15.22(02) & 15.10(03) & 14.72(14) & 13.77(13) & \nodata & AGN & 0.31 \\
g343 & 42.959742 & 60.592608 & \nodata & \nodata & \nodata & 14.42(01) & 13.71(01) & 12.96(04) & 11.88(04) & 8.99(11) & AGN & 0.14 \\
g344 & 42.962389 & 60.301164 & 15.68(07) & 15.27(09) & 14.94(12) & 14.83(02) & 14.83(03) & 14.66(13) & 14.29(17) & \nodata & AGN & 0.60 \\
g345 & 42.963552 & 60.230295 & 15.89(09) & 15.21(11) & 15.00(14) & 14.93(13) & 14.90(14) & 14.17(15) & 13.97(16) & \nodata & AGN & 0.58 \\
g346 & 42.965476 & 60.009964 & 14.99(05) & 14.21(04) & 13.98(05) & 13.83(02) & 13.84(02) & 13.98(15) & 12.85(18) & \nodata & PAH & 0.00 \\
g347 & 42.966061 & 60.163086 & \nodata & \nodata & 15.18(15) & 14.04(02) & 13.60(02) & 13.03(04) & 11.89(04) & 8.30(06) & AGN & 0.48 \\
g348 & 42.971163 & 60.351343 & \nodata & \nodata & \nodata & 15.98(08) & 14.92(04) & 14.10(11) & 12.23(04) & 9.26(26) & AGN & 0.03 \\
g349 & 42.975669 & 60.258365 & 16.75(14) & 16.01(19) & 15.64(23) & 15.23(02) & 14.91(03) & 14.54(10) & 13.68(10) & \nodata & AGN & 0.56 \\
g350 & 42.977793 & 59.635626 & \nodata & \nodata & \nodata & 15.11(04) & 14.98(04) & 14.45(15) & 11.61(04) & 9.03(10) & PAH & 0.00 \\
g351 & 42.978113 & 60.402978 & 15.80(08) & 14.93(07) & 14.75(12) & 14.51(01) & 14.42(02) & 14.46(09) & 13.88(10) & \nodata & AGN & 0.76 \\
g352 & 42.978590 & 59.732627 & \nodata & \nodata & \nodata & 16.42(05) & 15.45(04) & 14.52(10) & 13.17(08) & 8.75(06) & AGN & 0.00 \\
g353 & 42.979502 & 60.534816 & \nodata & \nodata & \nodata & 15.04(02) & 14.69(03) & 14.32(12) & 13.31(09) & \nodata & AGN & 0.64 \\
g354 & 42.981167 & 60.736075 & \nodata & \nodata & \nodata & 15.48(03) & 15.01(04) & 14.38(19) & 12.92(16) & \nodata & AGN & 0.02 \\
g355 & 42.982609 & 60.124806 & 16.55(14) & 15.90(17) & 15.38(18) & 15.11(04) & 14.67(04) & 14.14(12) & 13.37(18) & \nodata & AGN & 0.64 \\
g356 & 42.986458 & 60.491157 & \nodata & \nodata & \nodata & 15.18(03) & 14.96(04) & 14.70(14) & 14.04(18) & \nodata & AGN & 0.58 \\
g357 & 42.988900 & 60.123940 & 16.85(17) & 16.13(21) & 15.11(13) & 14.51(03) & 13.94(02) & 13.33(07) & 12.32(06) & \nodata & AGN & 0.45 \\
g358 & 43.000714 & 60.172881 & \nodata & \nodata & \nodata & 15.41(03) & 15.12(03) & 14.57(12) & 13.87(12) & \nodata & AGN & 0.29 \\
g359 & 43.000993 & 60.501827 & \nodata & \nodata & \nodata & 15.57(03) & 15.16(03) & 14.63(17) & 14.01(17) & \nodata & AGN & 0.32 \\
g360 & 43.003711 & 59.666083 & 15.85(08) & 15.09(09) & 14.78(10) & 14.65(02) & 14.52(02) & 14.44(11) & 13.84(13) & \nodata & AGN & 0.08 \\
g361 & 43.007881 & 60.190171 & \nodata & \nodata & \nodata & 15.77(03) & 15.27(04) & 14.88(13) & 13.99(13) & \nodata & AGN & 0.11 \\
g362 & 43.008352 & 59.501106 & \nodata & \nodata & \nodata & 15.16(02) & 15.08(04) & 13.76(07) & 11.78(03) & 9.17(14) & PAH & 0.00 \\
g363 & 43.011923 & 60.600649 & \nodata & \nodata & \nodata & 15.75(05) & 14.90(04) & 13.69(08) & 12.31(10) & \nodata & AGN & 0.03 \\
g364 & 43.011944 & 60.502427 & 15.89(07) & 15.26(10) & 14.78(11) & 14.36(01) & 14.32(02) & 14.39(12) & 13.82(11) & \nodata & AGN & 0.76 \\
g365 & 43.014853 & 60.385015 & 15.82(06) & 15.00(07) & 14.58(09) & 14.29(02) & 14.04(02) & 13.38(05) & 12.46(04) & 9.85(17) & AGN & 0.51 \\
g366 & 43.016051 & 60.537955 & 15.63(07) & 14.82(06) & 14.70(10) & 14.29(01) & 14.09(02) & 13.76(05) & 12.73(06) & 8.89(09) & AGN & 0.68 \\
g367 & 43.019361 & 59.352465 & \nodata & \nodata & \nodata & 14.88(03) & 14.67(04) & 14.32(16) & 11.76(04) & \nodata & PAH & 0.00 \\
g368 & 43.023605 & 59.529696 & \nodata & \nodata & \nodata & 14.99(02) & 14.87(03) & 14.67(17) & 13.21(08) & \nodata & PAH & 0.00 \\
g369 & 43.028520 & 59.600373 & 15.91(10) & 15.12(10) & 14.87(14) & 14.44(02) & 14.43(03) & 14.12(11) & 13.54(16) & \nodata & AGN & 0.35 \\
g370 & 43.028821 & 60.641434 & \nodata & \nodata & \nodata & 15.64(06) & 15.38(06) & 14.57(16) & 13.59(14) & \nodata & AGN & 0.02 \\
g371 & 43.039597 & 60.402605 & 16.17(09) & 15.26(12) & 14.95(12) & 14.41(02) & 14.22(02) & 13.81(07) & 12.77(05) & 9.37(14) & AGN & 0.56 \\
g372 & 43.040431 & 59.434018 & 15.48(05) & 14.78(07) & 14.53(08) & 14.28(02) & 14.29(02) & 14.36(09) & 13.75(10) & \nodata & AGN & 0.31 \\
g373 & 43.042342 & 60.744258 & \nodata & \nodata & \nodata & 14.43(02) & 13.96(02) & 13.27(09) & 12.50(19) & 7.77(14) & AGN & 0.25 \\
g374 & 43.045743 & 60.551302 & \nodata & \nodata & \nodata & 15.03(03) & 14.79(03) & 14.53(12) & 13.68(15) & \nodata & AGN & 0.47 \\
g375 & 43.048038 & 60.361632 & \nodata & \nodata & \nodata & 15.39(03) & 14.64(02) & 13.78(05) & 12.90(07) & 9.00(16) & AGN & 0.40 \\
g376 & 43.048897 & 60.258436 & 16.07(08) & 15.43(12) & 14.92(13) & 14.83(02) & 14.75(03) & 14.59(11) & 13.17(06) & 8.35(06) & PAH & 0.00 \\
g377 & 43.049489 & 60.246303 & 15.54(08) & 14.80(08) & 14.50(10) & 14.41(02) & 14.46(03) & 14.48(15) & 13.82(12) & \nodata & AGN & 0.43 \\
g378 & 43.056139 & 60.488544 & 15.91(09) & 15.22(10) & 14.94(12) & 14.60(02) & 14.61(03) & 14.51(10) & 14.11(14) & \nodata & AGN & 0.60 \\
g379 & 43.061835 & 60.312479 & \nodata & \nodata & \nodata & 16.57(06) & 15.49(05) & 14.79(12) & 13.41(08) & \nodata & AGN & 0.01 \\
g380 & 43.062033 & 59.540367 & 15.09(04) & 14.61(06) & 14.57(09) & 14.39(02) & 14.41(02) & 14.23(11) & 13.70(15) & \nodata & AGN & 0.37 \\
g381 & 43.063428 & 59.695297 & 15.63(06) & 15.25(10) & 15.12(13) & 14.87(02) & 14.60(03) & 14.08(07) & 12.44(04) & 9.64(09) & PAH & 0.00 \\
g382 & 43.073238 & 59.786410 & 15.63(06) & 14.99(08) & 14.68(09) & 14.74(02) & 14.68(03) & 14.49(12) & 13.55(15) & \nodata & AGN & 0.16 \\
g383 & 43.074730 & 60.627823 & \nodata & \nodata & \nodata & 16.32(08) & 15.27(06) & 14.51(19) & 12.95(12) & 9.35(15) & AGN & 0.01 \\
g384 & 43.080044 & 59.540200 & \nodata & \nodata & \nodata & 16.17(06) & 15.58(05) & 14.66(12) & 13.74(17) & \nodata & AGN & 0.00 \\
g385 & 43.089486 & 59.508515 & \nodata & \nodata & \nodata & 15.11(03) & 14.60(03) & 14.43(16) & 11.39(03) & 8.05(12) & PAH & 0.00 \\
g386 & 43.095652 & 60.570912 & \nodata & \nodata & \nodata & 14.75(03) & 14.23(02) & 13.83(08) & 12.72(09) & 9.65(20) & AGN & 0.51 \\
g387 & 43.101159 & 60.430652 & 15.65(06) & 15.01(07) & 14.48(09) & 14.36(01) & 14.32(02) & 14.23(10) & 13.67(14) & \nodata & AGN & 0.63 \\
g388 & 43.103681 & 60.569669 & \nodata & \nodata & \nodata & 14.54(02) & 14.03(02) & 13.55(07) & 12.65(10) & 9.38(20) & AGN & 0.68 \\
g389 & 43.115615 & 60.626974 & \nodata & \nodata & \nodata & 15.04(04) & 14.51(04) & 14.56(17) & 13.28(18) & 7.11(04) & PAH & 0.00 \\
g390 & 43.130769 & 60.488203 & \nodata & \nodata & \nodata & 15.22(04) & 15.00(04) & 14.53(16) & 13.97(15) & \nodata & AGN & 0.32 \\
g391 & 43.134887 & 60.140513 & \nodata & \nodata & \nodata & 15.64(04) & 15.18(03) & 14.54(13) & 13.93(15) & \nodata & AGN & 0.15 \\
g392 & 43.138058 & 60.544127 & 16.86(17) & 16.12(22) & 15.48(20) & 15.27(03) & 14.93(03) & 14.40(17) & 13.92(16) & \nodata & AGN & 0.59 \\
g393 & 43.138633 & 60.467244 & 16.78(17) & 16.12(20) & 15.56(22) & 14.68(02) & 14.21(02) & 13.88(08) & 12.85(07) & 9.21(14) & AGN & 0.68 \\
g394 & 43.139920 & 60.577229 & \nodata & \nodata & \nodata & 16.17(07) & 15.18(04) & 14.40(16) & 13.52(18) & 9.57(17) & AGN & 0.22 \\
g395 & 43.141388 & 60.610253 & \nodata & \nodata & \nodata & 14.89(02) & 14.58(03) & 13.98(08) & 13.46(11) & \nodata & AGN & 0.57 \\
g396 & 43.141919 & 59.410334 & 14.17(03) & 13.68(04) & 13.47(04) & 13.41(01) & 13.42(02) & 9.37(01) & 13.60(11) & \nodata & PAH & 0.00 \\
g397 & 43.142865 & 60.348275 & \nodata & \nodata & \nodata & 15.20(02) & 14.91(03) & 14.94(16) & 13.96(10) & \nodata & AGN & 0.48 \\
g398 & 43.145271 & 61.084160 & \nodata & \nodata & \nodata & 16.78(10) & 15.52(06) & 14.43(12) & 13.51(19) & \nodata & AGN & 0.00 \\
g399 & 43.150016 & 59.559961 & 15.35(05) & 14.75(06) & 14.60(08) & 14.38(02) & 14.31(02) & 14.14(08) & 13.77(13) & \nodata & AGN & 0.08 \\
g400 & 43.152053 & 60.026711 & 15.77(07) & 14.92(09) & 14.74(11) & 14.84(02) & 14.95(03) & 14.76(16) & 14.03(16) & \nodata & AGN & 0.24 \\
g401 & 43.154183 & 60.356049 & 15.66(07) & 14.76(06) & 14.68(10) & 14.39(01) & 14.34(02) & 14.09(07) & 13.77(12) & \nodata & AGN & 0.63 \\
g402 & 43.155937 & 60.441797 & 15.27(05) & 14.66(06) & 14.45(09) & 14.42(01) & 14.41(02) & 14.55(13) & 13.70(07) & \nodata & AGN & 0.76 \\
g403 & 43.162062 & 60.101057 & \nodata & \nodata & \nodata & 15.38(04) & 15.12(04) & 14.72(18) & 11.96(03) & 9.36(11) & PAH & 0.00 \\
g404 & 43.162417 & 60.785095 & 14.07(03) & 13.64(04) & 13.41(04) & 13.45(02) & 13.37(01) & 13.35(12) & 12.16(08) & \nodata & PAH & 0.00 \\
g405 & 43.166951 & 60.996314 & 13.79(03) & 13.20(04) & 13.10(04) & 12.96(01) & 13.07(01) & 12.80(10) & 11.83(11) & \nodata & PAH & 0.14 \\
g406 & 43.168541 & 59.520116 & 15.32(05) & 15.02(07) & 14.83(10) & 14.88(02) & 14.71(03) & 14.64(15) & 14.05(15) & \nodata & AGN & 0.30 \\
g407 & 43.173319 & 61.230641 & 15.25(06) & 14.44(07) & 14.02(07) & 14.03(01) & 14.14(03) & 13.95(07) & 13.60(16) & \nodata & AGN & 0.18 \\
g408 & 43.174336 & 60.551269 & \nodata & \nodata & \nodata & 15.89(04) & 14.94(03) & 14.28(10) & 13.45(11) & \nodata & AGN & 0.55 \\
g409 & 43.174626 & 60.539645 & \nodata & \nodata & \nodata & 15.30(02) & 14.76(03) & 14.29(12) & 13.49(14) & \nodata & AGN & 0.55 \\
g410 & 43.175712 & 60.628853 & \nodata & \nodata & \nodata & 13.84(02) & 13.30(01) & 13.21(09) & 11.94(07) & 8.15(15) & PAH & 0.00 \\
g411 & 43.177491 & 60.385405 & 15.68(07) & 15.37(11) & 15.29(17) & 14.74(02) & 14.69(03) & 14.65(12) & 14.08(12) & \nodata & AGN & 0.60 \\
g412 & 43.182395 & 60.315174 & 16.98(18) & 15.83(16) & 15.15(14) & 14.72(02) & 14.54(02) & 14.08(07) & 13.43(11) & \nodata & AGN & 0.57 \\
g413 & 43.182619 & 60.550644 & \nodata & \nodata & \nodata & 14.64(02) & 14.02(01) & 13.37(06) & 12.29(07) & 8.52(07) & AGN & 0.53 \\
g414 & 43.187071 & 60.416013 & 16.48(12) & 15.61(14) & 15.26(17) & 15.24(02) & 15.22(03) & 15.08(18) & 13.80(10) & \nodata & PAH & 0.00 \\
g415 & 43.188889 & 60.518516 & \nodata & \nodata & \nodata & 15.64(05) & 15.14(04) & 14.81(18) & 13.78(18) & \nodata & AGN & 0.29 \\
g416 & 43.188967 & 60.527578 & 17.19(24) & 15.61(13) & 14.92(12) & 14.43(01) & 14.08(02) & 13.96(08) & 13.56(18) & \nodata & AGN & 0.80 \\
g417 & 43.192965 & 60.554065 & \nodata & \nodata & \nodata & 15.40(03) & 15.00(03) & 14.46(14) & 13.66(12) & \nodata & AGN & 0.55 \\
g418 & 43.194097 & 60.486498 & \nodata & \nodata & \nodata & 14.98(02) & 14.55(02) & 14.05(07) & 13.32(06) & \nodata & AGN & 0.68 \\
g419 & 43.195202 & 60.442174 & \nodata & \nodata & \nodata & 15.53(04) & 14.69(03) & 14.08(08) & 13.05(06) & 9.71(13) & AGN & 0.48 \\
g420 & 43.196842 & 60.099092 & 15.50(06) & 15.12(09) & 15.02(13) & 14.73(02) & 14.75(03) & 14.70(15) & 14.02(13) & \nodata & AGN & 0.35 \\
g421 & 43.203229 & 60.417308 & 16.23(11) & 15.48(15) & 15.30(16) & 14.48(01) & 14.29(02) & 13.96(07) & 13.76(11) & \nodata & AGN & 0.63 \\
g422 & 43.203850 & 60.510057 & 16.08(08) & 15.26(09) & 15.11(15) & 14.67(02) & 14.62(03) & 14.62(13) & 14.03(20) & \nodata & AGN & 0.72 \\
g423 & 43.205154 & 60.805393 & \nodata & \nodata & \nodata & 14.72(02) & 14.38(02) & 14.68(20) & 13.65(14) & \nodata & PAH & 0.00 \\
g424 & 43.208052 & 60.283916 & \nodata & \nodata & \nodata & 15.49(03) & 14.71(03) & 13.78(06) & 12.32(04) & 8.27(05) & AGN & 0.02 \\
g425 & 43.217392 & 60.065893 & 15.60(07) & 15.13(09) & 15.08(15) & 14.75(02) & 14.77(04) & 14.87(18) & 14.24(18) & \nodata & AGN & 0.28 \\
g426 & 43.222517 & 60.402651 & \nodata & \nodata & \nodata & 14.87(02) & 14.26(02) & 13.79(06) & 12.93(07) & 9.88(14) & AGN & 0.56 \\
g427 & 43.226229 & 60.887180 & \nodata & \nodata & \nodata & 14.69(02) & 14.48(02) & 14.05(07) & 11.30(03) & 8.93(09) & PAH & 0.00 \\
g428 & 43.227421 & 59.439645 & 15.16(04) & 14.50(05) & 14.40(07) & 14.27(01) & 14.28(02) & 14.24(09) & 13.74(12) & \nodata & AGN & 0.08 \\
g429 & 43.228153 & 60.465582 & \nodata & \nodata & \nodata & 14.99(04) & 14.44(03) & 14.07(10) & 13.61(10) & \nodata & AGN & 0.74 \\
g430 & 43.239724 & 60.045543 & \nodata & \nodata & \nodata & 14.84(06) & 14.46(04) & 13.97(11) & 11.47(02) & 8.56(06) & PAH & 0.00 \\
g431 & 43.243407 & 60.529510 & 16.51(13) & 15.87(16) & 15.24(17) & 14.70(02) & 14.69(03) & 14.81(20) & 13.77(19) & \nodata & PAH & 0.00 \\
g432 & 43.249007 & 60.332804 & \nodata & \nodata & \nodata & 15.26(03) & 14.43(03) & 13.53(07) & 12.80(09) & 8.87(16) & AGN & 0.42 \\
g433 & 43.250176 & 60.580761 & 16.45(12) & \nodata & \nodata & 14.76(02) & 14.46(02) & 14.20(10) & 13.54(12) & \nodata & AGN & 0.61 \\
g434 & 43.256549 & 60.881198 & 15.16(05) & 14.84(07) & 14.59(10) & 14.30(01) & 14.23(02) & 14.16(10) & 13.67(18) & \nodata & AGN & 0.41 \\
g435 & 43.257430 & 60.251832 & \nodata & \nodata & \nodata & 16.35(06) & 15.43(05) & 14.71(13) & 13.85(12) & \nodata & AGN & 0.05 \\
g436 & 43.263882 & 60.270715 & 15.28(05) & 14.79(07) & 14.77(10) & 14.69(01) & 14.72(02) & 14.60(11) & 14.15(15) & \nodata & AGN & 0.41 \\
g437 & 43.267314 & 60.678847 & \nodata & \nodata & \nodata & 15.25(03) & 14.74(03) & 14.17(12) & 13.12(12) & 9.35(16) & AGN & 0.27 \\
g438 & 43.271273 & 60.529131 & 14.82(03) & 14.56(06) & 14.40(08) & 14.41(02) & 14.36(02) & 14.21(09) & 13.85(19) & \nodata & AGN & 0.63 \\
g439 & 43.272377 & 60.638417 & 16.70(15) & 16.04(19) & 15.04(14) & 14.92(02) & 14.70(03) & 14.24(13) & 13.28(18) & 9.90(24) & AGN & 0.36 \\
g440 & 43.275554 & 60.660061 & \nodata & \nodata & \nodata & 16.27(07) & 15.23(04) & 14.20(15) & 12.87(17) & \nodata & AGN & 0.01 \\
g441 & 43.277335 & 61.141187 & 15.94(08) & 15.05(10) & 15.01(14) & 14.71(02) & 14.68(02) & 14.43(14) & 13.59(18) & \nodata & AGN & 0.33 \\
g442 & 43.277664 & 60.447195 & \nodata & \nodata & \nodata & 15.57(04) & 14.78(03) & 13.84(05) & 12.75(06) & 9.08(09) & AGN & 0.07 \\
g443 & 43.289570 & 59.699516 & 15.55(05) & 14.97(08) & 14.81(10) & 14.69(02) & 14.56(02) & 14.45(11) & 13.96(16) & \nodata & AGN & 0.17 \\
g444 & 43.292957 & 60.174061 & 15.35(06) & 14.94(08) & 14.72(11) & 14.70(02) & 14.71(03) & 14.77(12) & 14.19(16) & \nodata & AGN & 0.35 \\
g445 & 43.295380 & 60.384541 & 16.84(16) & 16.05(22) & 15.74(26) & 14.85(02) & 14.38(02) & 13.87(07) & 13.05(09) & 10.14(16) & AGN & 0.56 \\
g446 & 43.315923 & 60.063680 & \nodata & \nodata & \nodata & 15.13(03) & 14.96(04) & 14.76(18) & 13.34(08) & \nodata & PAH & 0.00 \\
g447 & 43.316524 & 59.882036 & 16.08(09) & 15.15(10) & 15.04(14) & 14.79(02) & 14.77(03) & 14.48(13) & 13.74(20) & \nodata & AGN & 0.06 \\
g448 & 43.320667 & 59.991221 & 15.05(04) & 14.34(05) & 14.22(07) & 14.17(01) & 14.19(02) & 14.06(08) & 13.52(11) & \nodata & AGN & 0.37 \\
g449 & 43.328793 & 60.370211 & \nodata & \nodata & \nodata & 15.24(05) & 14.90(04) & 14.46(16) & 13.82(18) & 9.48(12) & AGN & 0.32 \\
g450 & 43.331129 & 61.072594 & 15.18(04) & 14.20(05) & 13.76(06) & 13.41(01) & 13.09(01) & 13.36(11) & 11.93(09) & \nodata & PAH & 0.00 \\
g451 & 43.339913 & 60.462769 & \nodata & \nodata & \nodata & 15.38(04) & 14.89(04) & 14.55(13) & 12.65(08) & 8.71(09) & PAH & 0.00 \\
g452 & 43.346296 & 60.383586 & 15.65(06) & 15.09(08) & 15.08(14) & 14.94(02) & 14.89(03) & 14.83(14) & 14.31(19) & \nodata & AGN & 0.34 \\
g453 & 43.354197 & 60.622704 & 16.26(10) & 15.08(10) & 14.89(12) & 14.40(01) & 14.21(02) & 13.91(06) & 13.59(11) & \nodata & AGN & 0.64 \\
g454 & 43.358939 & 60.396591 & \nodata & \nodata & \nodata & 15.23(04) & 15.04(05) & 14.57(15) & 13.73(16) & \nodata & AGN & 0.17 \\
g455 & 43.360304 & 61.214850 & \nodata & \nodata & \nodata & 15.36(03) & 14.64(03) & 13.91(09) & 12.69(07) & 8.68(07) & AGN & 0.08 \\
g456 & 43.362481 & 60.548465 & 16.42(11) & 16.02(17) & 15.22(16) & 14.66(01) & 14.46(02) & 14.12(06) & 13.70(10) & \nodata & AGN & 0.42 \\
g457 & 43.365282 & 60.682264 & \nodata & \nodata & \nodata & 15.17(02) & 14.81(03) & 14.37(12) & 13.30(12) & \nodata & AGN & 0.40 \\
g458 & 43.368153 & 60.583519 & 16.76(15) & 15.65(12) & 15.26(18) & 14.83(02) & 14.61(02) & 14.28(10) & 13.69(09) & \nodata & AGN & 0.58 \\
g459 & 43.368403 & 60.017731 & 15.49(06) & 14.91(08) & 14.71(10) & 14.78(01) & 14.82(02) & 14.61(12) & 14.06(14) & \nodata & AGN & 0.28 \\
g460 & 43.372388 & 60.296498 & \nodata & \nodata & \nodata & 15.23(02) & 14.99(04) & 14.41(11) & 13.31(09) & 9.72(13) & AGN & 0.33 \\
g461 & 43.373258 & 60.191699 & 16.73(16) & 15.71(14) & 15.22(16) & 14.94(02) & 14.61(02) & 14.24(09) & 13.95(10) & \nodata & AGN & 0.35 \\
g462 & 43.373268 & 59.681491 & \nodata & \nodata & \nodata & 15.42(03) & 14.60(02) & 14.04(10) & 12.92(07) & 8.87(07) & AGN & 0.20 \\
g463 & 43.386437 & 60.604271 & \nodata & \nodata & \nodata & 14.78(02) & 14.22(02) & 13.34(05) & 12.52(05) & 8.62(09) & AGN & 0.42 \\
g464 & 43.392429 & 60.513519 & \nodata & \nodata & \nodata & 15.78(03) & 15.01(03) & 14.37(11) & 13.13(06) & 10.00(19) & AGN & 0.04 \\
g465 & 43.401843 & 60.664552 & 16.50(14) & 15.56(13) & 15.34(18) & 14.80(02) & 14.53(02) & 14.44(13) & 13.61(18) & \nodata & AGN & 0.73 \\
g466 & 43.405262 & 60.265374 & \nodata & \nodata & \nodata & 15.46(03) & 14.95(03) & 14.40(10) & 13.61(10) & 10.24(20) & AGN & 0.30 \\
g467 & 43.407220 & 60.753783 & \nodata & \nodata & \nodata & 15.44(03) & 15.28(04) & 14.77(18) & 12.12(05) & \nodata & PAH & 0.00 \\
g468 & 43.411929 & 61.103772 & \nodata & \nodata & \nodata & 14.77(03) & 14.28(02) & 13.53(11) & 11.54(09) & 8.36(14) & PAH & 0.00 \\
g469 & 43.418028 & 60.882143 & \nodata & \nodata & \nodata & 15.04(04) & 14.38(03) & 13.80(13) & 12.70(20) & 8.82(15) & AGN & 0.12 \\
g470 & 43.419943 & 60.204845 & \nodata & \nodata & \nodata & 14.68(03) & 14.54(04) & 14.63(12) & 12.62(06) & \nodata & PAH & 0.00 \\
g471 & 43.421080 & 60.657829 & \nodata & \nodata & \nodata & 15.38(03) & 14.78(03) & 14.07(07) & 13.07(07) & \nodata & AGN & 0.41 \\
g472 & 43.425312 & 60.653920 & 16.14(10) & 15.05(10) & 14.66(10) & 14.64(02) & 14.54(02) & 14.58(12) & 13.75(14) & \nodata & AGN & 0.73 \\
g473 & 43.426165 & 60.253463 & \nodata & \nodata & \nodata & 14.76(02) & 13.83(01) & 12.95(04) & 11.96(04) & 8.15(05) & AGN & 0.09 \\
g474 & 43.426635 & 59.996032 & \nodata & \nodata & \nodata & 15.10(03) & 14.68(03) & 14.02(08) & 12.60(08) & 8.11(05) & AGN & 0.05 \\
g475 & 43.428379 & 60.697849 & \nodata & \nodata & \nodata & 15.58(03) & 15.13(05) & 14.70(15) & 14.41(19) & \nodata & AGN & 0.34 \\
g476 & 43.434730 & 60.662504 & 16.48(12) & 15.57(14) & \nodata & 15.30(03) & 15.27(05) & 15.05(16) & 14.08(19) & \nodata & AGN & 0.12 \\
g477 & 43.434767 & 61.172698 & 15.88(08) & 15.14(09) & 14.85(12) & 14.75(02) & 14.69(02) & 14.68(15) & 13.78(10) & \nodata & AGN & 0.34 \\
g478 & 43.443317 & 60.626153 & \nodata & \nodata & \nodata & 15.18(03) & 14.73(03) & 14.18(11) & 13.21(15) & \nodata & AGN & 0.48 \\
g479 & 43.443755 & 59.904248 & 14.93(04) & 14.43(06) & 14.38(07) & 14.32(02) & 14.25(03) & 14.45(14) & 13.65(15) & \nodata & AGN & 0.37 \\
g480 & 43.444130 & 60.658109 & \nodata & \nodata & \nodata & 15.19(02) & 14.99(04) & 14.83(15) & 13.95(17) & \nodata & AGN & 0.59 \\
g481 & 43.445543 & 60.784716 & 16.12(09) & 15.08(09) & 14.82(10) & 14.49(02) & 14.30(02) & 14.39(15) & 12.90(09) & 8.87(11) & PAH & 0.00 \\
g482 & 43.446777 & 60.344466 & 15.19(05) & 14.81(07) & 14.62(10) & 14.59(03) & 14.56(02) & 14.64(14) & 13.83(09) & \nodata & AGN & 0.60 \\
g483 & 43.449558 & 60.311435 & 14.96(04) & 14.65(07) & 14.55(09) & 14.40(02) & 14.42(02) & 14.41(11) & 13.90(16) & \nodata & AGN & 0.76 \\
g484 & 43.452724 & 60.637834 & 16.99(19) & 15.71(14) & 15.51(22) & 14.81(02) & 14.55(02) & 14.40(11) & 13.67(10) & \nodata & AGN & 0.73 \\
g485 & 43.453216 & 60.068801 & \nodata & \nodata & 14.27(09) & 14.08(01) & 14.20(02) & 14.04(08) & 13.66(11) & \nodata & AGN & 0.32 \\
g486 & 43.455986 & 60.648995 & 16.70(14) & 15.62(15) & 15.39(19) & 14.62(02) & 14.22(02) & 13.68(08) & 12.83(05) & \nodata & AGN & 0.71 \\
g487 & 43.459780 & 60.314303 & \nodata & \nodata & \nodata & 16.50(07) & 15.31(04) & 14.29(10) & 13.21(11) & 9.84(17) & AGN & 0.01 \\
g488 & 43.460183 & 60.356282 & \nodata & \nodata & \nodata & 16.33(06) & 15.58(05) & 14.55(14) & 13.65(10) & \nodata & AGN & 0.00 \\
g489 & 43.461828 & 61.246456 & \nodata & \nodata & \nodata & 15.01(03) & 14.03(03) & 12.99(05) & 12.01(04) & 8.39(06) & AGN & 0.05 \\
g490 & 43.463102 & 59.696248 & \nodata & \nodata & 15.15(13) & 14.17(01) & 13.56(01) & 12.86(04) & 11.52(05) & 7.78(04) & AGN & 0.04 \\
g491 & 43.463686 & 60.694873 & \nodata & \nodata & \nodata & 14.85(02) & 14.47(03) & 14.39(14) & 13.88(16) & \nodata & AGN & 0.76 \\
g492 & 43.465162 & 59.986990 & \nodata & \nodata & \nodata & 15.32(02) & 15.17(03) & 14.60(15) & 13.18(08) & \nodata & PAH & 0.00 \\
g493 & 43.470799 & 60.620709 & \nodata & \nodata & \nodata & 15.34(02) & 14.99(03) & 14.69(18) & 13.64(15) & \nodata & AGN & 0.53 \\
g494 & 43.474914 & 60.739884 & \nodata & \nodata & \nodata & 15.74(04) & 15.21(04) & 14.37(11) & 13.35(12) & 9.26(12) & AGN & 0.05 \\
g495 & 43.477095 & 61.163368 & \nodata & \nodata & \nodata & 15.74(04) & 15.16(05) & 14.42(16) & 13.50(12) & 9.69(15) & AGN & 0.11 \\
g496 & 43.477964 & 60.606469 & 15.86(06) & 15.31(10) & 15.14(13) & 14.87(02) & 14.88(03) & 14.70(19) & 13.64(12) & \nodata & PAH & 0.00 \\
g497 & 43.480459 & 61.041226 & 15.13(04) & 14.63(05) & 14.43(08) & 14.19(02) & 14.14(02) & 13.57(09) & 12.44(14) & \nodata & AGN & 0.06 \\
g498 & 43.486289 & 61.076961 & 15.19(04) & 14.65(06) & 14.37(08) & 14.25(01) & 14.27(02) & 14.23(11) & 13.73(12) & \nodata & AGN & 0.18 \\
g499 & 43.495268 & 59.621609 & \nodata & \nodata & \nodata & 15.36(03) & 15.14(04) & 14.49(11) & 13.97(15) & \nodata & AGN & 0.15 \\
g500 & 43.497382 & 60.578276 & \nodata & \nodata & \nodata & 15.98(04) & 15.27(04) & 14.65(16) & 13.68(10) & \nodata & AGN & 0.07 \\
g501 & 43.497550 & 60.659142 & \nodata & \nodata & \nodata & 14.51(02) & 13.95(02) & 13.54(08) & 12.50(08) & 8.97(14) & AGN & 0.62 \\
g502 & 43.499882 & 61.002913 & 15.79(07) & 14.86(07) & 14.48(09) & 14.05(02) & 14.00(02) & 13.47(09) & 12.21(15) & \nodata & PAH & 0.00 \\
g503 & 43.501266 & 60.647862 & 16.01(07) & 15.28(09) & 15.15(16) & 14.47(01) & 14.36(02) & 14.21(10) & 13.76(13) & \nodata & AGN & 0.79 \\
g504 & 43.509379 & 59.954196 & \nodata & \nodata & \nodata & 16.98(07) & 15.89(07) & 14.77(13) & 13.37(08) & 9.70(12) & AGN & 0.00 \\
g505 & 43.511520 & 60.304211 & \nodata & \nodata & \nodata & 15.73(04) & 14.87(04) & 14.01(07) & 13.03(08) & 9.72(12) & AGN & 0.12 \\
g506 & 43.512530 & 60.644188 & 16.16(09) & 15.24(10) & 14.73(11) & 14.78(02) & 14.66(03) & 14.45(12) & 13.19(06) & 8.18(07) & PAH & 0.00 \\
g507 & 43.514141 & 60.553725 & \nodata & \nodata & \nodata & 15.03(04) & 14.63(04) & 14.47(20) & 13.92(12) & \nodata & AGN & 0.41 \\
g508 & 43.514870 & 60.662730 & 16.45(14) & 15.55(14) & 15.56(22) & 14.85(03) & 14.49(03) & 14.39(10) & 13.68(10) & \nodata & AGN & 0.78 \\
g509 & 43.515740 & 59.959602 & 16.57(13) & \nodata & \nodata & 15.36(02) & 15.21(03) & 15.21(19) & 13.50(08) & \nodata & PAH & 0.01 \\
g510 & 43.516164 & 60.796518 & \nodata & \nodata & \nodata & 15.38(03) & 14.50(02) & 13.47(07) & 12.35(08) & 8.43(11) & AGN & 0.05 \\
g511 & 43.516702 & 59.881827 & 15.15(05) & 14.56(07) & 14.49(09) & 14.38(01) & 14.30(02) & 14.17(10) & 13.65(19) & \nodata & AGN & 0.31 \\
g512 & 43.518886 & 59.684663 & \nodata & 15.60(13) & 15.12(13) & 14.16(01) & 13.87(02) & 13.56(07) & 10.61(02) & 7.83(08) & PAH & 0.00 \\
g513 & 43.521415 & 59.772064 & 15.61(07) & \nodata & 14.70(09) & 14.39(01) & 14.36(02) & 14.50(09) & 13.85(10) & \nodata & AGN & 0.31 \\
g514 & 43.525432 & 60.672480 & 15.93(08) & 14.87(09) & 14.57(10) & 14.46(03) & 14.43(03) & 14.45(12) & 13.72(09) & 9.11(08) & AGN & 0.80 \\
g515 & 43.526457 & 60.257741 & \nodata & \nodata & \nodata & 15.10(03) & 14.67(03) & 14.66(19) & 13.43(10) & \nodata & PAH & 0.00 \\
g516 & 43.528801 & 60.457392 & 16.69(15) & 15.64(14) & 15.14(14) & 14.86(03) & 14.73(03) & 14.16(10) & 13.22(08) & 10.06(15) & AGN & 0.27 \\
g517 & 43.529215 & 60.700975 & \nodata & \nodata & \nodata & 15.25(04) & 14.58(03) & 13.90(07) & 13.12(07) & \nodata & AGN & 0.64 \\
g518 & 43.529695 & 60.658123 & \nodata & \nodata & \nodata & 16.34(08) & 15.43(05) & 14.28(10) & 12.99(09) & 7.20(20) & AGN & 0.01 \\
g519 & 43.532883 & 60.660510 & \nodata & \nodata & \nodata & 15.05(04) & 14.49(03) & 13.89(08) & 13.07(08) & \nodata & AGN & 0.71 \\
g520 & 43.537445 & 60.276154 & 16.82(17) & 15.77(15) & 15.55(20) & 15.19(03) & 15.06(03) & 14.60(18) & 13.73(12) & \nodata & AGN & 0.25 \\
g521 & 43.539230 & 60.667291 & 16.30(11) & 15.14(13) & 15.01(15) & 14.48(02) & 14.15(03) & 13.83(13) & 12.82(07) & \nodata & AGN & 0.71 \\
g522 & 43.540862 & 60.662456 & \nodata & \nodata & \nodata & 15.25(02) & 14.91(04) & 14.43(17) & 13.73(13) & \nodata & AGN & 0.59 \\
g523 & 43.567376 & 60.182177 & \nodata & \nodata & \nodata & 15.03(02) & 14.71(03) & 14.22(09) & 11.56(03) & 8.56(08) & PAH & 0.00 \\
g524 & 43.569585 & 60.635490 & 15.44(06) & 14.45(06) & 13.97(06) & 13.89(01) & 13.61(01) & 13.09(04) & 12.06(05) & \nodata & AGN & 0.46 \\
g525 & 43.570416 & 60.503824 & \nodata & \nodata & \nodata & 15.33(02) & 14.96(03) & 14.77(14) & 14.12(19) & \nodata & AGN & 0.48 \\
g526 & 43.577180 & 60.650707 & 14.49(06) & 13.75(06) & 13.47(05) & 13.21(01) & 13.16(01) & 12.70(04) & 11.41(03) & 7.03(20) & PAH & 0.00 \\
g527 & 43.578294 & 60.439347 & 15.34(05) & 14.55(06) & 14.34(07) & 14.28(01) & 14.39(03) & 14.49(11) & 13.82(17) & \nodata & AGN & 0.43 \\
g528 & 43.582705 & 60.330136 & \nodata & \nodata & \nodata & 15.63(05) & 15.18(04) & 14.55(12) & 13.88(14) & \nodata & AGN & 0.17 \\
g529 & 43.582779 & 60.198034 & \nodata & \nodata & \nodata & 15.42(03) & 14.85(03) & 14.09(09) & 13.29(10) & \nodata & AGN & 0.16 \\
g530 & 43.584266 & 60.669399 & 16.65(13) & 15.62(14) & 15.12(14) & 14.83(03) & 14.67(03) & 14.36(10) & 13.82(13) & \nodata & AGN & 0.73 \\
g531 & 43.585958 & 60.499261 & \nodata & \nodata & \nodata & 14.90(02) & 14.33(02) & 13.87(06) & 12.76(04) & 9.27(11) & AGN & 0.42 \\
g532 & 43.590335 & 59.523162 & \nodata & \nodata & \nodata & 14.67(02) & 13.75(01) & 12.84(03) & 11.81(04) & 7.98(15) & AGN & 0.09 \\
g533 & 43.593588 & 59.639151 & 14.73(04) & 14.35(04) & 14.14(05) & 14.09(01) & 14.05(02) & 14.16(08) & 13.53(11) & \nodata & AGN & 0.32 \\
g534 & 43.594464 & 60.969797 & \nodata & \nodata & \nodata & 14.90(03) & 14.69(03) & 14.58(19) & 12.55(07) & 10.09(14) & PAH & 0.00 \\
g535 & 43.605475 & 60.747579 & 15.36(05) & 14.96(08) & 14.63(09) & 14.61(01) & 14.56(02) & 14.41(13) & 13.96(16) & \nodata & AGN & 0.41 \\
g536 & 43.605807 & 60.673766 & \nodata & \nodata & \nodata & 14.92(02) & 14.57(02) & 14.29(10) & 13.66(08) & \nodata & AGN & 0.70 \\
g537 & 43.613553 & 61.302350 & \nodata & \nodata & \nodata & 14.78(02) & 14.18(02) & 13.53(06) & 12.20(05) & 9.02(08) & AGN & 0.04 \\
g538 & 43.616778 & 60.594628 & \nodata & \nodata & \nodata & 14.88(02) & 14.55(02) & 14.16(07) & 13.50(09) & \nodata & AGN & 0.57 \\
g539 & 43.618153 & 60.522298 & \nodata & \nodata & \nodata & 16.16(05) & 15.60(05) & 14.82(20) & 12.49(06) & 9.79(14) & PAH & 0.00 \\
g540 & 43.620158 & 60.491168 & 14.95(05) & 14.45(05) & 14.29(07) & 14.23(01) & 14.21(02) & 14.14(09) & 13.69(12) & \nodata & AGN & 0.77 \\
g541 & 43.628010 & 59.985287 & 15.59(04) & 14.90(06) & 14.66(07) & 14.32(01) & 14.32(02) & 14.10(08) & 13.60(10) & \nodata & AGN & 0.37 \\
g542 & 43.628981 & 61.207507 & \nodata & \nodata & \nodata & 14.95(02) & 14.68(03) & 14.27(10) & 11.19(02) & 8.20(09) & PAH & 0.00 \\
g543 & 43.632018 & 59.687427 & 14.91(04) & 14.48(06) & 14.37(06) & 14.27(01) & 14.21(02) & 14.17(10) & 13.61(17) & \nodata & AGN & 0.37 \\
g544 & 43.633797 & 60.658970 & 16.67(14) & 16.30(27) & 15.35(18) & 15.10(02) & 14.97(03) & 14.72(15) & 13.52(18) & \nodata & AGN & 0.53 \\
g545 & 43.639883 & 60.503414 & \nodata & \nodata & \nodata & 15.71(04) & 15.40(06) & 14.44(14) & 13.67(15) & \nodata & AGN & 0.08 \\
g546 & 43.646757 & 61.237899 & \nodata & \nodata & \nodata & 15.18(03) & 14.42(02) & 13.52(07) & 12.33(07) & 8.06(05) & AGN & 0.04 \\
g547 & 43.653513 & 60.622960 & 15.90(08) & 14.98(07) & 14.59(10) & 14.31(01) & 13.94(02) & 13.36(05) & 12.47(06) & \nodata & AGN & 0.60 \\
g548 & 43.658438 & 59.564802 & \nodata & \nodata & \nodata & 15.30(04) & 14.49(03) & 13.98(09) & 13.04(07) & \nodata & AGN & 0.15 \\
g549 & 43.659017 & 60.834183 & \nodata & \nodata & \nodata & 15.42(03) & 14.36(03) & 13.31(05) & 12.39(07) & 9.18(09) & AGN & 0.09 \\
g550 & 43.659731 & 59.896684 & \nodata & \nodata & \nodata & 15.64(08) & 15.07(05) & 14.59(12) & 13.46(09) & 9.34(12) & AGN & 0.09 \\
g551 & 43.662682 & 60.475238 & 16.73(16) & \nodata & \nodata & 15.05(02) & 14.65(03) & 14.35(11) & 13.26(11) & \nodata & AGN & 0.53 \\
g552 & 43.666280 & 60.702526 & \nodata & \nodata & \nodata & 15.36(03) & 14.35(02) & 13.32(05) & 12.20(04) & 8.81(11) & AGN & 0.09 \\
g553 & 43.666829 & 61.197046 & \nodata & \nodata & \nodata & 14.89(03) & 14.71(04) & 13.77(08) & 11.31(02) & 8.79(08) & PAH & 0.00 \\
g554 & 43.667377 & 60.673629 & \nodata & \nodata & \nodata & 15.28(03) & 14.55(03) & 14.03(07) & 12.94(07) & 8.56(07) & AGN & 0.50 \\
g555 & 43.672169 & 60.884840 & \nodata & \nodata & \nodata & 14.97(02) & 14.53(02) & 14.19(11) & 13.13(15) & \nodata & AGN & 0.07 \\
g556 & 43.680264 & 60.647709 & 16.40(11) & 15.42(11) & 15.05(14) & 14.72(02) & 14.43(03) & 13.83(09) & 12.78(12) & \nodata & AGN & 0.52 \\
g557 & 43.682768 & 60.737260 & 16.21(10) & 15.49(12) & 15.04(14) & 14.41(02) & 14.32(02) & 13.82(08) & 12.63(12) & 9.39(17) & AGN & 0.29 \\
g558 & 43.684547 & 61.137428 & \nodata & \nodata & \nodata & 15.31(04) & 15.14(06) & 14.42(15) & 11.91(06) & 8.58(11) & PAH & 0.00 \\
g559 & 43.692386 & 60.837064 & 15.74(07) & 15.04(08) & 15.19(15) & 14.86(02) & 14.84(03) & 14.49(09) & 13.90(14) & \nodata & AGN & 0.28 \\
g560 & 43.692490 & 60.577992 & 15.63(10) & 15.30(12) & 14.43(10) & 14.58(02) & 13.94(01) & 13.29(04) & 12.13(04) & 9.10(09) & AGN & 0.14 \\
g561 & 43.693089 & 60.634949 & \nodata & \nodata & \nodata & 14.94(03) & 14.32(02) & 13.87(07) & 12.78(06) & 10.81(94) & AGN & 0.50 \\
g562 & 43.693200 & 60.640829 & \nodata & \nodata & \nodata & 14.88(02) & 14.70(03) & 14.26(12) & 13.78(11) & \nodata & AGN & 0.70 \\
g563 & 43.696211 & 60.015321 & \nodata & \nodata & \nodata & 15.80(04) & 15.15(05) & 14.31(15) & 13.14(17) & 8.63(09) & AGN & 0.02 \\
g564 & 43.696936 & 60.700363 & \nodata & \nodata & \nodata & 15.63(04) & 15.29(05) & 14.52(18) & 13.22(19) & \nodata & AGN & 0.02 \\
g565 & 43.701960 & 60.203738 & \nodata & \nodata & \nodata & 15.35(03) & 14.38(02) & 13.76(06) & 12.75(06) & 9.74(14) & AGN & 0.21 \\
g566 & 43.702395 & 60.478706 & \nodata & \nodata & \nodata & 16.86(07) & 15.59(04) & 14.18(08) & 12.91(06) & 9.62(10) & AGN & 0.00 \\
g567 & 43.703307 & 61.268449 & \nodata & \nodata & \nodata & 16.58(07) & 15.64(05) & 14.72(16) & 13.96(15) & \nodata & AGN & 0.00 \\
g568 & 43.709803 & 61.215884 & \nodata & \nodata & \nodata & 15.74(05) & 15.30(05) & 14.50(14) & 13.50(11) & 10.22(17) & AGN & 0.01 \\
g569 & 43.720611 & 59.939858 & \nodata & \nodata & \nodata & 15.66(03) & 15.21(04) & 14.89(13) & 12.22(03) & 9.50(09) & PAH & 0.00 \\
g570 & 43.721480 & 60.345996 & \nodata & \nodata & \nodata & 14.94(03) & 14.76(03) & 14.22(15) & 13.86(20) & \nodata & AGN & 0.28 \\
g571 & 43.725117 & 60.371254 & 16.37(12) & 15.80(16) & 15.33(17) & 14.83(02) & 14.56(02) & 14.19(12) & 12.92(07) & 9.69(14) & AGN & 0.23 \\
g572 & 43.727019 & 61.114955 & \nodata & \nodata & \nodata & 15.14(03) & 14.38(02) & 14.00(13) & 11.52(06) & 7.62(05) & PAH & 0.00 \\
g573 & 43.728187 & 60.919787 & 17.00(20) & 15.68(15) & 14.92(12) & 14.13(02) & 13.95(02) & 14.13(17) & 13.08(18) & \nodata & PAH & 0.28 \\
g574 & 43.729163 & 60.181725 & \nodata & \nodata & \nodata & 15.06(03) & 14.36(03) & 13.88(08) & 12.27(04) & 7.83(05) & PAH & 0.00 \\
g575 & 43.729341 & 59.722968 & \nodata & \nodata & \nodata & 15.21(03) & 14.38(02) & 13.51(06) & 12.27(05) & 8.91(07) & AGN & 0.04 \\
g576 & 43.729799 & 60.668120 & 16.53(13) & 15.50(12) & \nodata & 14.12(02) & 13.71(02) & 13.22(10) & 11.98(18) & 8.72(11) & AGN & 0.46 \\
g577 & 43.744304 & 60.351180 & 15.99(09) & 15.41(11) & 15.16(15) & 14.75(02) & 14.57(03) & 14.57(18) & 13.14(17) & \nodata & PAH & 0.00 \\
g578 & 43.745151 & 60.837828 & \nodata & \nodata & \nodata & 15.32(04) & 14.82(04) & 14.49(20) & 12.78(15) & 9.14(15) & PAH & 0.00 \\
g579 & 43.746789 & 60.351008 & \nodata & \nodata & \nodata & 14.97(02) & 14.52(03) & 14.28(16) & 12.58(08) & 8.78(17) & PAH & 0.00 \\
g580 & 43.747546 & 60.678710 & 16.81(15) & 15.89(16) & 15.47(20) & 14.83(02) & 14.51(02) & 13.64(09) & 12.63(13) & \nodata & AGN & 0.17 \\
g581 & 43.750954 & 60.558003 & \nodata & \nodata & \nodata & 16.27(05) & 15.35(04) & 14.22(10) & 13.44(11) & 9.50(12) & AGN & 0.01 \\
g582 & 43.756640 & 59.935592 & 16.89(21) & 15.63(15) & 14.90(13) & 14.21(02) & 13.70(02) & 12.92(03) & 11.45(03) & 8.26(08) & AGN & 0.02 \\
g583 & 43.785137 & 59.700549 & \nodata & \nodata & \nodata & 15.52(03) & 14.44(03) & 13.54(05) & 12.50(05) & 9.03(13) & AGN & 0.07 \\
g584 & 43.788120 & 60.569268 & 16.42(12) & 15.59(12) & 15.15(15) & 14.75(02) & 14.61(03) & 14.40(12) & 13.51(12) & 8.99(11) & AGN & 0.32 \\
g585 & 43.798117 & 60.704398 & \nodata & \nodata & \nodata & 14.37(04) & 13.60(02) & 13.14(07) & 11.66(13) & 7.59(20) & AGN & 0.10 \\
g586 & 43.802992 & 60.441281 & 16.56(12) & 15.86(16) & \nodata & 14.79(02) & 14.57(02) & 14.30(10) & 13.79(15) & \nodata & AGN & 0.34 \\
g587 & 43.807216 & 60.671197 & 16.38(10) & 15.39(10) & 15.03(13) & 14.20(01) & 13.83(02) & 13.06(04) & 11.94(05) & \nodata & AGN & 0.09 \\
g588 & 43.809551 & 60.261856 & \nodata & \nodata & \nodata & 14.90(02) & 14.50(02) & 14.28(10) & 13.25(10) & \nodata & AGN & 0.30 \\
g589 & 43.821511 & 60.151963 & \nodata & 15.94(18) & 15.12(15) & 14.31(01) & 13.92(01) & 13.33(05) & 10.73(02) & 8.18(06) & PAH & 0.00 \\
g590 & 43.822006 & 59.982336 & 14.97(04) & 14.36(06) & 14.15(07) & 14.05(01) & 14.10(01) & 14.08(07) & 13.55(10) & \nodata & AGN & 0.37 \\
g591 & 43.829986 & 60.225715 & \nodata & 15.96(18) & 15.10(14) & 14.63(04) & 14.10(03) & 13.62(14) & 12.17(18) & \nodata & AGN & 0.09 \\
g592 & 43.830188 & 60.829542 & \nodata & \nodata & \nodata & 15.16(02) & 14.90(03) & 14.31(14) & 11.92(06) & 8.33(08) & PAH & 0.00 \\
g593 & 43.838225 & 60.826671 & \nodata & \nodata & \nodata & 14.81(02) & 14.68(03) & 14.09(08) & 11.48(04) & \nodata & PAH & 0.00 \\
g594 & 43.843068 & 61.164325 & \nodata & 15.66(13) & 14.96(13) & 14.62(02) & 14.24(02) & 13.82(09) & 12.69(09) & \nodata & AGN & 0.21 \\
g595 & 43.847471 & 60.818146 & \nodata & \nodata & 14.88(13) & 14.49(02) & 14.26(02) & 14.20(10) & 11.38(04) & 8.95(10) & PAH & 0.00 \\
g596 & 43.848060 & 59.963930 & \nodata & \nodata & \nodata & 15.76(03) & 15.35(03) & 14.94(16) & 13.55(08) & \nodata & AGN & 0.01 \\
g597 & 43.855885 & 60.740692 & 15.09(05) & 14.45(05) & 14.14(06) & 13.94(01) & 13.97(02) & 13.73(10) & 12.67(15) & \nodata & PAH & 0.36 \\
g598 & 43.856460 & 60.119505 & 15.40(06) & 14.86(07) & 14.56(09) & 14.44(01) & 14.47(03) & 14.07(11) & 13.94(16) & \nodata & AGN & 0.31 \\
g599 & 43.858071 & 60.207807 & 15.78(06) & 14.90(07) & 14.81(11) & 14.32(02) & 14.11(02) & 13.85(07) & 12.60(06) & 8.62(06) & AGN & 0.24 \\
g600 & 43.859618 & 61.109171 & \nodata & \nodata & \nodata & 16.41(07) & 15.32(05) & 14.10(14) & 12.97(09) & 9.23(17) & AGN & 0.00 \\
g601 & 43.862238 & 60.745545 & 14.49(04) & 13.82(04) & 13.73(05) & 13.53(01) & 13.59(01) & 13.33(08) & 12.26(05) & \nodata & PAH & 0.36 \\
g602 & 43.870362 & 60.900600 & \nodata & \nodata & \nodata & 15.67(04) & 14.84(03) & 13.84(10) & 12.76(16) & 9.19(13) & AGN & 0.04 \\
g603 & 43.872770 & 60.304479 & 16.06(15) & 15.32(14) & 14.86(13) & 14.46(02) & 14.01(02) & 13.46(07) & 12.51(07) & 9.12(09) & AGN & 0.25 \\
g604 & 43.883772 & 59.876256 & \nodata & \nodata & \nodata & 16.48(06) & 15.49(04) & 14.62(10) & 13.55(09) & \nodata & AGN & 0.01 \\
g605 & 43.888055 & 60.840562 & 16.10(10) & 15.31(12) & 14.53(09) & 14.64(01) & 14.67(03) & 14.54(12) & 13.48(10) & 9.53(14) & PAH & 0.46 \\
g606 & 43.894385 & 61.331938 & \nodata & \nodata & \nodata & 15.96(05) & 14.77(03) & 13.95(08) & 12.46(05) & \nodata & AGN & 0.00 \\
g607 & 43.896684 & 60.021167 & \nodata & \nodata & \nodata & 15.17(03) & 14.85(03) & 14.63(13) & 11.55(02) & 8.58(07) & PAH & 0.00 \\
g608 & 43.911645 & 59.761770 & \nodata & \nodata & \nodata & 15.65(04) & 15.29(04) & 14.39(14) & 13.63(12) & \nodata & AGN & 0.03 \\
g609 & 43.912550 & 61.198581 & \nodata & \nodata & \nodata & 15.01(03) & 14.36(03) & 13.22(06) & 11.83(04) & 7.45(04) & AGN & 0.00 \\
g610 & 43.919407 & 60.467244 & 14.91(04) & 14.29(05) & 14.11(07) & 13.97(01) & 13.98(02) & 13.85(12) & 12.73(12) & \nodata & PAH & 0.00 \\
g611 & 43.926844 & 59.903407 & \nodata & \nodata & \nodata & 16.03(04) & 15.05(03) & 14.06(09) & 12.37(07) & 7.73(09) & AGN & 0.01 \\
g612 & 43.927473 & 60.896325 & 13.40(03) & 12.99(04) & 12.74(03) & 12.60(01) & 12.53(01) & 11.60(03) & 9.97(04) & 6.21(13) & PAH & 0.00 \\
g613 & 43.929418 & 60.289718 & \nodata & \nodata & \nodata & 15.27(04) & 15.02(04) & 14.79(12) & 14.19(13) & \nodata & AGN & 0.15 \\
g614 & 43.958107 & 60.294239 & \nodata & \nodata & \nodata & 14.71(02) & 14.56(02) & 13.73(06) & 11.21(03) & 7.70(06) & PAH & 0.00 \\
g615 & 43.977183 & 60.186885 & 16.38(12) & 15.39(12) & 15.13(17) & 14.45(01) & 14.09(02) & 13.50(05) & 12.70(08) & \nodata & AGN & 0.32 \\
g616 & 43.979475 & 60.174816 & \nodata & \nodata & \nodata & 15.47(04) & 14.99(04) & 14.67(19) & 13.78(13) & \nodata & AGN & 0.32 \\
g617 & 43.984552 & 60.524255 & \nodata & \nodata & 15.12(18) & 14.40(07) & 14.19(06) & 13.52(12) & 10.92(07) & 7.17(08) & PAH & 0.00 \\
g618 & 43.991225 & 60.488552 & \nodata & \nodata & \nodata & 15.98(05) & 15.02(03) & 13.97(10) & 12.38(09) & \nodata & AGN & 0.00 \\
g619 & 43.997620 & 61.351064 & \nodata & \nodata & \nodata & 15.85(04) & 14.89(04) & 14.21(12) & 13.17(08) & 9.06(10) & AGN & 0.04 \\
g620 & 44.003543 & 59.769960 & 15.55(05) & 14.73(05) & 14.65(07) & 14.40(01) & 14.40(02) & 14.46(12) & 13.64(12) & \nodata & AGN & 0.08 \\
g621 & 44.008043 & 60.104535 & 15.07(04) & 14.72(06) & 14.66(10) & 14.48(01) & 14.43(02) & 14.48(10) & 13.84(15) & \nodata & AGN & 0.31 \\
g622 & 44.014914 & 59.694736 & 16.32(10) & 16.02(14) & 15.77(20) & 15.27(03) & 14.75(03) & 13.89(09) & 12.90(10) & \nodata & AGN & 0.04 \\
g623 & 44.025225 & 61.091871 & \nodata & \nodata & 15.12(16) & 14.28(01) & 13.80(01) & 13.36(06) & 12.29(06) & 8.83(14) & AGN & 0.24 \\
g624 & 44.036340 & 60.383337 & \nodata & \nodata & \nodata & 15.28(04) & 14.63(03) & 13.91(14) & 12.44(20) & 7.70(10) & AGN & 0.04 \\
g625 & 44.038998 & 60.229030 & 15.54(06) & 14.94(07) & 14.54(10) & 14.40(01) & 14.36(02) & 13.84(07) & 13.64(11) & \nodata & AGN & 0.37 \\
g626 & 44.054195 & 60.211521 & \nodata & \nodata & \nodata & 16.12(04) & 15.82(04) & 14.74(11) & 13.77(14) & 8.42(06) & AGN & 0.00 \\
g627 & 44.067164 & 60.721780 & 13.64(03) & 12.78(03) & 12.42(03) & 12.19(01) & 12.17(01) & 12.04(10) & 10.84(10) & \nodata & PAH & 0.00 \\
g628 & 44.067885 & 60.202932 & \nodata & \nodata & \nodata & 14.98(03) & 14.55(03) & 14.33(14) & 12.19(10) & 9.17(08) & PAH & 0.00 \\
g629 & 44.071428 & 60.361961 & \nodata & \nodata & \nodata & 15.71(04) & 14.93(05) & 14.29(12) & 12.70(17) & \nodata & AGN & 0.01 \\
g630 & 44.081752 & 60.868501 & \nodata & \nodata & \nodata & 14.99(03) & 14.81(03) & 14.06(16) & 11.56(07) & 8.29(07) & PAH & 0.00 \\
g631 & 44.085139 & 60.327385 & 16.36(12) & 15.63(16) & 15.00(15) & 14.79(02) & 14.56(02) & 14.41(09) & 13.91(10) & \nodata & AGN & 0.30 \\
g632 & 44.090388 & 60.091600 & 15.71(07) & 15.26(09) & 15.10(16) & 14.78(01) & 14.77(03) & 14.67(14) & 14.01(16) & \nodata & AGN & 0.24 \\
g633 & 44.104708 & 61.120907 & \nodata & \nodata & \nodata & 15.50(05) & 15.20(07) & 14.73(18) & 11.96(04) & 9.56(20) & PAH & 0.00 \\
g634 & 44.131036 & 61.269847 & \nodata & \nodata & \nodata & 16.06(05) & 15.33(04) & 14.55(14) & 13.45(10) & \nodata & AGN & 0.00 \\
g635 & 44.137328 & 59.924677 & \nodata & \nodata & \nodata & 15.68(05) & 14.74(03) & 13.88(11) & 12.26(12) & 8.24(16) & AGN & 0.01 \\
g636 & 44.151865 & 59.887249 & \nodata & \nodata & \nodata & 14.31(03) & 14.10(04) & 13.72(11) & 10.86(04) & 8.22(14) & PAH & 0.00 \\
g637 & 44.152341 & 59.739950 & 14.57(03) & 14.18(04) & 14.09(05) & 14.05(01) & 14.11(02) & 13.91(09) & 13.61(13) & \nodata & AGN & 0.18 \\
g638 & 44.152469 & 61.324742 & \nodata & \nodata & \nodata & 16.15(06) & 15.22(04) & 14.46(13) & 13.35(10) & \nodata & AGN & 0.04 \\
g639 & 44.169485 & 61.308958 & \nodata & \nodata & \nodata & 15.90(04) & 15.16(04) & 14.27(12) & 13.36(09) & 9.31(11) & AGN & 0.04 \\
g640 & 44.186920 & 60.950695 & \nodata & \nodata & \nodata & 14.95(03) & 14.71(03) & 14.35(15) & 11.33(05) & 8.90(16) & PAH & 0.00 \\
g641 & 44.187002 & 59.875196 & \nodata & \nodata & \nodata & 16.25(07) & 15.00(04) & 14.07(10) & 12.61(08) & \nodata & AGN & 0.00 \\
g642 & 44.199919 & 60.290936 & 15.02(05) & 14.69(08) & 14.52(10) & 14.33(01) & 14.35(02) & 14.29(10) & 13.17(16) & \nodata & PAH & 0.04 \\
g643 & 44.204035 & 60.633363 & 16.14(10) & 15.17(09) & 14.89(12) & 14.34(02) & 14.02(02) & 13.43(10) & 11.96(11) & \nodata & AGN & 0.02 \\
g644 & 44.239057 & 60.128438 & 15.29(05) & 14.82(09) & 14.56(12) & 14.42(02) & 14.41(03) & 13.86(13) & 13.03(17) & \nodata & AGN & 0.07 \\
g645 & 44.252133 & 61.383006 & \nodata & \nodata & \nodata & 15.37(03) & 14.81(03) & 14.59(16) & 13.44(10) & \nodata & AGN & 0.06 \\
g646 & 44.274050 & 60.960967 & \nodata & \nodata & \nodata & 14.99(03) & 14.63(03) & 14.22(12) & 13.24(17) & \nodata & AGN & 0.34 \\
g647 & 44.301364 & 60.420664 & 15.71(06) & 14.96(07) & 15.00(13) & 14.73(02) & 14.56(02) & 13.98(15) & 12.60(17) & \nodata & AGN & 0.02 \\
g648 & 44.308766 & 61.144175 & \nodata & \nodata & \nodata & 15.02(03) & 14.83(03) & 14.29(15) & 12.01(05) & 9.02(19) & PAH & 0.00 \\
g649 & 44.312161 & 60.101814 & \nodata & \nodata & \nodata & 14.10(08) & 13.50(08) & 12.99(18) & 11.35(12) & 7.54(06) & PAH & 0.00 \\
g650 & 44.321240 & 60.876571 & \nodata & \nodata & \nodata & 14.66(03) & 14.45(03) & 13.77(19) & 11.27(11) & 8.00(19) & PAH & 0.00 \\
g651 & 44.330937 & 60.436490 & \nodata & \nodata & \nodata & 14.71(03) & 13.87(02) & 13.31(09) & 11.82(09) & 7.78(11) & AGN & 0.01 \\
g652 & 44.332187 & 60.272299 & \nodata & \nodata & \nodata & 16.07(06) & 15.22(04) & 14.25(14) & 12.82(20) & \nodata & AGN & 0.00 \\
g653 & 44.336184 & 61.305878 & \nodata & \nodata & \nodata & 16.33(06) & 15.33(05) & 14.57(15) & 13.32(09) & 9.80(22) & AGN & 0.01 \\
g654 & 44.342159 & 61.371045 & \nodata & \nodata & \nodata & 15.32(03) & 14.69(04) & 13.80(09) & 13.21(10) & \nodata & AGN & 0.07 \\
g655 & 44.347303 & 61.144357 & \nodata & 15.18(12) & 14.39(09) & 13.81(01) & 13.62(01) & 13.29(05) & 11.48(04) & 9.33(10) & PAH & 0.00 \\
g656 & 44.353530 & 60.574142 & \nodata & \nodata & \nodata & 15.18(04) & 14.91(04) & 14.53(18) & 12.06(11) & \nodata & PAH & 0.00 \\
g657 & 44.358692 & 60.585357 & \nodata & \nodata & \nodata & 15.00(03) & 14.23(02) & 13.38(08) & 11.85(12) & 8.06(10) & AGN & 0.02 \\
g658 & 44.359965 & 59.634710 & \nodata & \nodata & \nodata & 15.11(02) & 14.49(02) & 13.87(08) & 12.62(05) & \nodata & AGN & 0.07 \\
g659 & 44.370213 & 60.563933 & 15.74(09) & 14.98(09) & 14.78(13) & 13.96(02) & 13.72(02) & 13.21(08) & 12.14(15) & \nodata & AGN & 0.22 \\
g660 & 44.383012 & 59.900573 & 15.89(06) & 15.29(08) & 15.14(11) & 14.86(02) & 14.64(02) & 14.59(14) & 13.01(10) & \nodata & PAH & 0.00 \\
g661 & 44.405027 & 60.063167 & 16.30(12) & 16.00(20) & 15.39(19) & 15.00(03) & 15.02(04) & 14.08(12) & 13.12(18) & \nodata & AGN & 0.03 \\
g662 & 44.410655 & 60.957115 & \nodata & \nodata & \nodata & 15.09(02) & 14.71(03) & 14.31(12) & 11.84(06) & 8.96(10) & PAH & 0.00 \\
g663 & 44.419178 & 60.632628 & \nodata & \nodata & \nodata & 14.67(04) & 14.10(02) & 13.41(08) & 12.12(15) & \nodata & AGN & 0.11 \\
g664 & 44.420003 & 60.642338 & \nodata & \nodata & \nodata & 14.82(02) & 14.20(02) & 13.26(07) & 12.19(07) & \nodata & AGN & 0.05 \\
g665 & 44.420803 & 60.081624 & \nodata & \nodata & \nodata & 14.72(03) & 14.58(04) & 13.80(11) & 11.34(05) & 8.45(12) & PAH & 0.00 \\
g666 & 44.421778 & 60.399012 & \nodata & \nodata & \nodata & 14.61(03) & 13.76(02) & 12.74(05) & 11.61(07) & \nodata & AGN & 0.04 \\
g667 & 44.436562 & 59.682439 & \nodata & \nodata & \nodata & 14.96(03) & 14.19(02) & 13.79(14) & 12.84(10) & \nodata & AGN & 0.33 \\
g668 & 44.442888 & 60.420875 & \nodata & \nodata & \nodata & 15.20(03) & 14.99(05) & 14.29(14) & 12.00(09) & 8.74(11) & PAH & 0.00 \\
g669 & 44.444851 & 60.433572 & \nodata & \nodata & \nodata & 14.80(03) & 14.31(02) & 13.60(10) & 12.31(12) & \nodata & AGN & 0.05 \\
g670 & 44.445029 & 60.975503 & \nodata & \nodata & \nodata & 16.03(06) & 15.44(05) & 14.73(15) & 13.79(18) & 9.69(13) & AGN & 0.01 \\
g671 & 44.447711 & 59.977381 & 16.02(09) & 15.25(11) & 14.83(11) & 14.68(02) & 14.72(03) & 14.83(16) & 14.03(16) & \nodata & AGN & 0.35 \\
g672 & 44.452293 & 60.314420 & \nodata & \nodata & \nodata & 15.68(15) & 15.07(10) & 13.90(18) & 12.60(12) & \nodata & AGN & 0.01 \\
g673 & 44.458572 & 61.085957 & \nodata & \nodata & \nodata & 16.17(06) & 15.54(05) & 14.60(18) & 13.52(19) & \nodata & AGN & 0.00 \\
g674 & 44.461450 & 59.664362 & 17.24(21) & 16.16(16) & 15.24(12) & 14.84(02) & 14.31(02) & 14.07(12) & 12.90(10) & \nodata & AGN & 0.32 \\
g675 & 44.474500 & 61.167340 & 15.74(08) & 14.97(09) & 14.84(12) & 14.58(02) & 14.54(02) & 14.56(16) & 13.88(19) & \nodata & AGN & 0.30 \\
g676 & 44.475504 & 60.593873 & 15.83(08) & 15.21(11) & 14.96(13) & 14.64(02) & 14.55(02) & 14.27(12) & 13.31(15) & \nodata & AGN & 0.57 \\
g677 & 44.476763 & 59.667548 & \nodata & \nodata & \nodata & 14.62(02) & 13.70(01) & 12.74(04) & 11.59(04) & \nodata & AGN & 0.04 \\
g678 & 44.486914 & 60.592299 & 15.95(09) & 15.04(12) & 14.63(11) & 14.17(01) & 13.95(01) & 13.81(09) & 12.64(09) & \nodata & PAH & 0.00 \\
g679 & 44.491200 & 59.856396 & 15.13(04) & 14.73(06) & 14.59(07) & 14.40(02) & 14.38(02) & 14.49(14) & 13.85(16) & \nodata & AGN & 0.08 \\
g680 & 44.497133 & 59.666580 & 16.17(07) & 15.38(08) & 15.04(10) & 14.37(02) & 13.64(01) & 13.06(06) & 12.03(06) & \nodata & AGN & 0.26 \\
g681 & 44.503926 & 60.639771 & 17.06(22) & 15.68(16) & 15.37(19) & 15.21(04) & 14.84(04) & 14.46(14) & 13.69(19) & \nodata & AGN & 0.32 \\
g682 & 44.508656 & 60.729795 & \nodata & \nodata & \nodata & 15.65(04) & 15.11(04) & 14.30(14) & 13.31(19) & 8.63(09) & AGN & 0.04 \\
g683 & 44.514639 & 60.602082 & 15.48(06) & 14.46(06) & 14.26(07) & 14.12(01) & 14.02(02) & 14.01(10) & 12.97(10) & 9.23(17) & PAH & 0.00 \\
g684 & 44.520879 & 60.258518 & \nodata & 14.96(08) & \nodata & 14.45(02) & 14.49(02) & 14.47(12) & 13.57(19) & \nodata & AGN & 0.36 \\
g685 & 44.522885 & 61.275603 & \nodata & \nodata & \nodata & 14.61(02) & 14.13(03) & 13.52(09) & 11.90(05) & 8.31(07) & AGN & 0.02 \\
g686 & 44.525154 & 60.000786 & \nodata & \nodata & \nodata & 15.94(05) & 15.24(04) & 14.59(14) & 13.58(17) & 9.96(25) & AGN & 0.10 \\
g687 & 44.525631 & 61.128044 & 15.33(07) & 14.80(09) & 14.56(11) & 14.41(02) & 14.33(02) & 14.24(12) & 13.82(17) & \nodata & AGN & 0.43 \\
g688 & 44.526736 & 60.563000 & \nodata & \nodata & \nodata & 15.84(06) & 14.74(03) & 14.17(10) & 13.09(13) & 9.33(14) & AGN & 0.23 \\
g689 & 44.535258 & 60.092295 & \nodata & \nodata & \nodata & 15.39(03) & 14.60(02) & 13.67(09) & 12.93(14) & 9.42(16) & AGN & 0.23 \\
g690 & 44.535774 & 59.897019 & \nodata & \nodata & \nodata & 16.02(05) & 15.25(03) & 14.37(10) & 13.36(11) & \nodata & AGN & 0.04 \\
g691 & 44.539143 & 60.771338 & 17.02(22) & 15.79(17) & 15.30(19) & 14.46(02) & 14.05(02) & 13.56(10) & 12.65(18) & \nodata & AGN & 0.07 \\
g692 & 44.548092 & 61.126673 & \nodata & \nodata & \nodata & 15.13(02) & 14.76(02) & 13.87(07) & 13.54(08) & \nodata & AGN & 0.47 \\
g693 & 44.549132 & 60.260162 & \nodata & \nodata & \nodata & 15.19(04) & 14.35(02) & 13.57(08) & 12.82(19) & \nodata & AGN & 0.24 \\
g694 & 44.551077 & 60.372793 & \nodata & \nodata & \nodata & 14.85(03) & 14.23(03) & 13.70(09) & 12.89(13) & \nodata & AGN & 0.39 \\
g695 & 44.552767 & 61.151544 & \nodata & 15.57(14) & 15.03(13) & 14.48(01) & 14.14(02) & 13.54(07) & 12.57(05) & 9.09(11) & AGN & 0.24 \\
g696 & 44.554303 & 59.570804 & \nodata & \nodata & \nodata & 14.84(03) & 14.06(02) & 13.23(08) & 12.58(09) & \nodata & AGN & 0.33 \\
g697 & 44.557111 & 59.549702 & \nodata & \nodata & \nodata & 14.86(03) & 13.90(02) & 12.99(05) & 11.93(05) & \nodata & AGN & 0.02 \\
g698 & 44.561650 & 60.179902 & \nodata & \nodata & \nodata & 16.08(04) & 15.85(05) & 15.23(18) & 13.37(09) & \nodata & PAH & 0.00 \\
g699 & 44.566529 & 60.443979 & 16.18(11) & 15.54(12) & 15.17(16) & 14.42(02) & 13.97(02) & 13.52(07) & 12.45(12) & 9.13(10) & AGN & 0.22 \\
g700 & 44.567048 & 59.613034 & \nodata & \nodata & \nodata & 16.33(08) & 15.07(06) & 13.84(12) & 11.23(04) & \nodata & PAH & 0.18 \\
g701 & 44.567288 & 60.074680 & \nodata & \nodata & \nodata & 15.46(05) & 14.93(04) & 14.79(17) & 13.09(15) & 9.05(17) & PAH & 0.00 \\
g702 & 44.570371 & 60.746366 & \nodata & \nodata & \nodata & 14.53(02) & 14.29(02) & 13.71(08) & 12.76(14) & \nodata & AGN & 0.21 \\
g703 & 44.588557 & 60.173910 & \nodata & \nodata & \nodata & 16.94(08) & 15.78(05) & 14.72(18) & 13.55(13) & 9.68(14) & AGN & 0.00 \\
g704 & 44.595850 & 59.982827 & \nodata & \nodata & \nodata & 16.26(05) & 15.30(03) & 14.31(10) & 13.23(09) & 9.45(22) & AGN & 0.01 \\
g705 & 44.597341 & 60.117556 & \nodata & \nodata & \nodata & 16.20(06) & 14.63(02) & 13.57(07) & 12.36(05) & 7.91(09) & AGN & 0.02 \\
g706 & 44.599759 & 60.632215 & \nodata & \nodata & \nodata & 14.97(02) & 14.46(02) & 14.05(11) & 13.12(11) & \nodata & AGN & 0.38 \\
g707 & 44.602658 & 61.076988 & \nodata & \nodata & \nodata & 15.47(04) & 15.07(03) & 14.57(15) & 13.11(12) & \nodata & AGN & 0.04 \\
g708 & 44.604472 & 60.313505 & \nodata & 15.44(12) & 15.29(17) & 14.52(02) & 14.32(02) & 13.93(08) & 13.04(15) & \nodata & AGN & 0.38 \\
g709 & 44.605151 & 60.133712 & \nodata & \nodata & \nodata & 16.20(04) & 15.52(05) & 14.37(12) & 13.18(14) & 9.73(25) & AGN & 0.00 \\
g710 & 44.619052 & 60.541291 & 16.03(10) & 15.15(11) & 14.94(14) & 14.58(02) & 14.39(02) & 14.40(11) & 13.39(16) & \nodata & PAH & 0.00 \\
g711 & 44.626223 & 59.637156 & \nodata & \nodata & \nodata & 15.59(05) & 14.66(04) & 13.67(09) & 12.93(10) & \nodata & AGN & 0.27 \\
g712 & 44.629609 & 60.633113 & 16.44(14) & 15.44(13) & 15.23(16) & 14.62(02) & 14.44(02) & 13.81(13) & 12.52(17) & 8.34(22) & AGN & 0.10 \\
g713 & 44.646159 & 60.401347 & \nodata & \nodata & \nodata & 15.48(03) & 15.16(04) & 14.52(17) & 13.66(19) & 9.61(20) & AGN & 0.25 \\
g714 & 44.647241 & 59.964862 & \nodata & \nodata & \nodata & 14.88(03) & 14.06(02) & 13.45(05) & 12.10(05) & 8.01(10) & AGN & 0.11 \\
g715 & 44.661705 & 59.693491 & 17.35(22) & 16.11(15) & 15.51(15) & 15.32(03) & 15.00(04) & 14.73(18) & 13.93(20) & \nodata & AGN & 0.27 \\
g716 & 44.663255 & 59.688232 & \nodata & 16.21(17) & 15.39(14) & 15.21(03) & 14.80(04) & 14.36(14) & 13.04(10) & \nodata & AGN & 0.07 \\
g717 & 44.664745 & 60.767637 & 16.50(17) & 15.27(11) & 15.34(20) & 14.46(02) & 14.10(02) & 13.61(08) & 12.50(12) & \nodata & AGN & 0.24 \\
g718 & 44.673856 & 60.589431 & 16.52(16) & 15.74(16) & 15.37(18) & 14.82(02) & 14.57(02) & 13.87(09) & 13.20(17) & \nodata & AGN & 0.53 \\
g719 & 44.678972 & 60.582090 & \nodata & \nodata & \nodata & 14.57(02) & 13.86(02) & 13.25(06) & 12.19(08) & 8.28(18) & AGN & 0.37 \\
g720 & 44.680104 & 60.138420 & 15.72(07) & 14.71(07) & 14.35(08) & 14.42(01) & 14.29(02) & 14.14(09) & 13.57(12) & 9.08(09) & AGN & 0.36 \\
g721 & 44.682803 & 60.789993 & \nodata & \nodata & 14.94(14) & 14.31(02) & 13.76(01) & 13.28(06) & 10.72(04) & 7.52(04) & PAH & 0.00 \\
g722 & 44.684652 & 60.320684 & \nodata & \nodata & \nodata & 15.93(05) & 14.90(03) & 13.61(09) & 12.27(12) & 8.64(13) & AGN & 0.03 \\
g723 & 44.686102 & 60.624205 & \nodata & \nodata & \nodata & 15.40(03) & 15.15(04) & 14.44(15) & 13.04(17) & \nodata & AGN & 0.05 \\
g724 & 44.701443 & 60.359967 & \nodata & \nodata & \nodata & 16.11(04) & 15.30(04) & 14.31(13) & 13.76(11) & 10.18(19) & AGN & 0.07 \\
g725 & 44.703492 & 59.644848 & \nodata & \nodata & \nodata & 15.63(04) & 14.88(03) & 14.12(16) & 13.16(16) & \nodata & AGN & 0.19 \\
g726 & 44.704453 & 59.908554 & \nodata & \nodata & \nodata & 14.70(02) & 14.05(02) & 13.40(05) & 12.45(04) & \nodata & AGN & 0.25 \\
g727 & 44.706122 & 60.276727 & \nodata & \nodata & \nodata & 15.75(04) & 15.37(04) & 14.81(17) & 13.56(10) & 9.82(11) & AGN & 0.01 \\
g728 & 44.706781 & 60.192395 & 15.44(07) & 14.99(08) & 14.53(08) & 14.61(02) & 14.61(02) & 14.73(17) & 14.10(19) & \nodata & AGN & 0.35 \\
g729 & 44.711703 & 60.365656 & 15.96(09) & 15.31(13) & 14.98(13) & 14.90(02) & 14.95(04) & 14.59(17) & 14.04(15) & \nodata & AGN & 0.48 \\
g730 & 44.719943 & 60.386901 & \nodata & \nodata & \nodata & 16.17(04) & 15.62(05) & 14.39(13) & 12.97(13) & \nodata & AGN & 0.00 \\
g731 & 44.723698 & 60.132067 & \nodata & \nodata & \nodata & 15.63(04) & 14.94(03) & 14.64(14) & 12.22(07) & 9.01(14) & PAH & 0.00 \\
g732 & 44.730874 & 59.923480 & \nodata & \nodata & \nodata & 15.57(03) & 15.29(04) & 14.29(10) & 13.06(08) & 7.80(12) & AGN & 0.01 \\
g733 & 44.744980 & 60.344424 & \nodata & \nodata & \nodata & 16.00(06) & 15.37(04) & 14.31(12) & 13.39(14) & 9.48(11) & AGN & 0.02 \\
g734 & 44.758089 & 60.428927 & \nodata & \nodata & \nodata & 15.88(04) & 15.49(05) & 14.84(14) & 13.08(06) & \nodata & PAH & 0.00 \\
g735 & 44.760651 & 59.946257 & \nodata & \nodata & \nodata & 16.53(05) & 15.25(04) & 14.18(08) & 12.98(07) & 9.34(21) & AGN & 0.00 \\
g736 & 44.764637 & 60.553617 & 16.58(16) & 15.53(15) & 15.10(15) & 14.66(02) & 14.35(02) & 14.13(09) & 13.69(17) & \nodata & AGN & 0.79 \\
g737 & 44.767797 & 60.621711 & \nodata & \nodata & \nodata & 14.75(02) & 14.54(03) & 14.26(13) & 13.67(18) & \nodata & AGN & 0.58 \\
g738 & 44.770869 & 60.009462 & \nodata & \nodata & \nodata & 16.51(12) & 15.46(05) & 14.41(10) & 13.36(10) & \nodata & AGN & 0.01 \\
g739 & 44.776004 & 60.622489 & \nodata & \nodata & \nodata & 15.19(03) & 14.95(04) & 14.44(11) & 13.32(11) & \nodata & AGN & 0.33 \\
g740 & 44.776779 & 60.562156 & 15.61(07) & 15.02(08) & 14.92(12) & 14.66(03) & 14.66(03) & 14.40(14) & 13.67(13) & \nodata & AGN & 0.73 \\
g741 & 44.779252 & 60.549637 & \nodata & \nodata & \nodata & 14.96(02) & 14.65(03) & 14.35(14) & 13.85(14) & \nodata & AGN & 0.73 \\
g742 & 44.779745 & 60.711043 & 14.90(04) & 14.42(06) & 14.28(08) & 14.09(01) & 14.03(02) & 13.89(07) & 13.53(10) & \nodata & AGN & 0.36 \\
g743 & 44.782650 & 60.410865 & \nodata & \nodata & \nodata & 15.27(03) & 15.03(03) & 14.44(14) & 11.88(05) & 9.25(09) & PAH & 0.00 \\
g744 & 44.787568 & 61.046024 & 16.06(11) & 15.22(11) & 14.82(12) & 14.58(02) & 14.51(03) & 14.24(16) & 13.72(18) & \nodata & AGN & 0.09 \\
g745 & 44.787884 & 60.563536 & \nodata & \nodata & \nodata & 15.29(02) & 15.05(04) & 14.51(12) & 13.70(12) & \nodata & AGN & 0.31 \\
g746 & 44.803630 & 60.571564 & 16.65(17) & 15.71(15) & 15.72(25) & 14.87(02) & 14.82(04) & 14.44(12) & 13.85(17) & \nodata & AGN & 0.60 \\
g747 & 44.808880 & 60.430972 & \nodata & \nodata & \nodata & 14.51(01) & 14.08(02) & 12.91(03) & 11.68(02) & 7.56(03) & AGN & 0.02 \\
g748 & 44.816672 & 60.690934 & 15.46(06) & 14.96(09) & 14.70(11) & 14.66(02) & 14.58(03) & 14.34(14) & 13.84(17) & \nodata & AGN & 0.41 \\
g749 & 44.819355 & 60.565783 & \nodata & \nodata & \nodata & 14.74(03) & 14.62(04) & 14.13(09) & 12.82(07) & \nodata & AGN & 0.18 \\
g750 & 44.821185 & 60.709467 & \nodata & \nodata & \nodata & 15.49(03) & 15.28(04) & 14.68(13) & 12.13(04) & \nodata & PAH & 0.00 \\
g751 & 44.823741 & 60.499325 & \nodata & \nodata & \nodata & 14.98(02) & 14.63(03) & 14.16(11) & 13.07(16) & \nodata & AGN & 0.48 \\
g752 & 44.824846 & 61.055965 & \nodata & \nodata & \nodata & 16.19(13) & 14.99(06) & 13.90(17) & 12.90(16) & 9.28(10) & AGN & 0.01 \\
g753 & 44.826411 & 60.406384 & \nodata & \nodata & \nodata & 14.88(02) & 14.58(02) & 14.09(09) & 13.46(14) & \nodata & AGN & 0.39 \\
g754 & 44.827096 & 60.464701 & \nodata & \nodata & \nodata & 14.64(02) & 14.24(02) & 14.04(07) & 13.54(15) & 9.27(13) & AGN & 0.77 \\
g755 & 44.827251 & 59.814840 & \nodata & \nodata & \nodata & 15.53(03) & 14.67(03) & 13.75(09) & 12.96(10) & \nodata & AGN & 0.11 \\
g756 & 44.830075 & 60.442155 & \nodata & \nodata & \nodata & 15.32(03) & 15.10(03) & 14.63(15) & 13.14(10) & 9.71(11) & PAH & 0.00 \\
g757 & 44.830655 & 60.681156 & \nodata & \nodata & \nodata & 15.82(04) & 15.19(04) & 14.57(17) & 12.45(07) & \nodata & PAH & 0.00 \\
g758 & 44.832875 & 59.624542 & \nodata & \nodata & \nodata & 15.24(05) & 14.21(03) & 13.38(08) & 12.38(07) & \nodata & AGN & 0.08 \\
g759 & 44.841501 & 60.604799 & 15.98(11) & 15.13(10) & 14.71(11) & 14.33(01) & 14.07(02) & 13.74(08) & 12.22(05) & 8.34(08) & PAH & 0.00 \\
g760 & 44.842462 & 60.501382 & \nodata & \nodata & \nodata & 15.67(07) & 14.94(05) & 14.00(08) & 12.91(07) & 9.55(17) & AGN & 0.08 \\
g761 & 44.843199 & 60.543773 & \nodata & \nodata & \nodata & 14.78(02) & 14.53(03) & 14.25(11) & 13.68(16) & \nodata & AGN & 0.73 \\
g762 & 44.845179 & 60.792787 & 14.78(04) & 14.13(05) & 14.21(08) & 13.97(02) & 13.99(02) & 13.52(10) & 12.50(13) & \nodata & AGN & 0.28 \\
g763 & 44.845906 & 60.536214 & \nodata & \nodata & \nodata & 15.90(06) & 15.01(05) & 13.95(08) & 12.90(09) & 9.13(10) & AGN & 0.05 \\
g764 & 44.846384 & 60.557135 & 16.45(16) & 15.53(15) & 15.49(23) & 15.11(04) & 14.85(04) & 14.32(13) & 13.78(15) & \nodata & AGN & 0.59 \\
g765 & 44.847177 & 60.358656 & \nodata & \nodata & \nodata & 15.60(03) & 15.14(03) & 14.38(14) & 12.03(04) & 7.73(05) & PAH & 0.00 \\
g766 & 44.850328 & 60.580892 & \nodata & \nodata & \nodata & 14.75(03) & 14.32(03) & 13.68(08) & 12.73(06) & \nodata & AGN & 0.52 \\
g767 & 44.851844 & 60.579465 & \nodata & 15.37(14) & \nodata & 14.10(01) & 14.00(03) & 14.06(16) & 12.79(10) & \nodata & PAH & 0.46 \\
g768 & 44.852213 & 60.494219 & 16.39(14) & 15.64(16) & 15.01(16) & 14.42(01) & 14.23(02) & 13.67(06) & 12.61(05) & \nodata & AGN & 0.53 \\
g769 & 44.852849 & 60.631196 & 16.79(21) & 15.65(17) & 15.28(19) & 14.51(01) & 14.16(02) & 13.85(06) & 13.57(12) & \nodata & AGN & 0.77 \\
g770 & 44.855073 & 60.576150 & \nodata & \nodata & \nodata & 14.41(02) & 13.82(02) & 13.64(08) & 12.36(04) & 7.91(04) & PAH & 0.00 \\
g771 & 44.855774 & 60.580525 & \nodata & \nodata & \nodata & 15.04(03) & 14.69(04) & 14.24(10) & 13.50(16) & \nodata & AGN & 0.71 \\
g772 & 44.859832 & 60.591941 & \nodata & \nodata & \nodata & 15.16(03) & 14.73(04) & 14.37(18) & 13.57(16) & \nodata & AGN & 0.71 \\
g773 & 44.862823 & 60.493092 & \nodata & \nodata & \nodata & 15.20(03) & 14.44(03) & 13.57(05) & 12.70(07) & \nodata & AGN & 0.52 \\
g774 & 44.865240 & 60.535524 & \nodata & \nodata & \nodata & 14.91(04) & 14.71(04) & 14.66(14) & 13.86(20) & \nodata & AGN & 0.70 \\
g775 & 44.867873 & 60.573909 & 16.71(21) & 15.70(18) & 15.41(22) & 14.64(03) & 14.41(05) & 13.83(10) & 12.87(12) & \nodata & AGN & 0.53 \\
g776 & 44.872051 & 60.871723 & \nodata & \nodata & \nodata & 14.98(02) & 14.80(03) & 14.32(13) & 12.28(05) & 10.37(40) & PAH & 0.00 \\
g777 & 44.872772 & 60.567683 & \nodata & \nodata & \nodata & 14.98(03) & 14.73(04) & 14.60(17) & 13.91(17) & \nodata & AGN & 0.73 \\
g778 & 44.873279 & 60.490669 & \nodata & \nodata & \nodata & 15.02(02) & 14.45(02) & 14.24(10) & 13.71(13) & \nodata & AGN & 0.79 \\
g779 & 44.874891 & 60.471544 & \nodata & \nodata & \nodata & 15.70(04) & 14.85(04) & 14.47(10) & 13.69(10) & \nodata & AGN & 0.56 \\
g780 & 44.881916 & 60.561491 & \nodata & \nodata & \nodata & 14.84(03) & 14.52(03) & 14.24(17) & 13.70(19) & \nodata & AGN & 0.73 \\
g781 & 44.883133 & 60.678466 & 16.55(16) & 15.42(12) & 15.19(17) & 14.69(02) & 14.42(02) & 14.12(11) & 12.86(08) & \nodata & AGN & 0.29 \\
g782 & 44.883831 & 60.598425 & 16.05(12) & 14.82(12) & 14.53(12) & 14.16(03) & 13.86(03) & 13.40(10) & 12.22(12) & \nodata & AGN & 0.47 \\
g783 & 44.884802 & 60.580689 & 16.14(12) & 15.10(12) & 14.66(12) & 14.51(02) & 14.47(02) & 14.63(12) & 13.90(17) & \nodata & AGN & 0.80 \\
g784 & 44.889029 & 60.642879 & 15.50(08) & 15.09(09) & 14.73(11) & 14.54(01) & 14.52(02) & 14.50(10) & 13.41(11) & \nodata & PAH & 0.46 \\
g785 & 44.896731 & 60.612795 & 16.20(12) & 15.60(16) & 14.78(12) & 14.40(01) & 14.19(02) & 13.86(08) & 12.73(08) & 9.28(17) & AGN & 0.71 \\
g786 & 44.899413 & 60.581108 & 16.38(14) & 15.23(11) & 14.99(16) & 14.51(02) & 14.13(02) & 13.59(05) & 12.47(07) & 9.30(13) & AGN & 0.54 \\
g787 & 44.900560 & 60.599019 & 15.41(06) & 14.56(07) & \nodata & 13.93(01) & 13.69(01) & 13.36(06) & 12.15(05) & 8.77(11) & AGN & 0.48 \\
g788 & 44.906023 & 60.593812 & \nodata & \nodata & \nodata & 15.33(03) & 15.04(03) & 14.81(17) & 13.66(15) & \nodata & AGN & 0.31 \\
g789 & 44.912027 & 60.586897 & \nodata & \nodata & \nodata & 15.37(03) & 15.07(04) & 14.38(10) & 13.31(10) & \nodata & AGN & 0.09 \\
g790 & 44.913334 & 60.548783 & \nodata & \nodata & \nodata & 15.32(03) & 14.87(04) & 14.80(18) & 13.43(14) & \nodata & PAH & 0.00 \\
g791 & 44.914775 & 60.613470 & \nodata & \nodata & \nodata & 15.89(04) & 14.79(03) & 13.44(05) & 12.55(05) & 9.30(11) & AGN & 0.09 \\
g792 & 44.923119 & 60.575132 & \nodata & \nodata & \nodata & 15.06(03) & 14.79(03) & 14.50(16) & 13.66(15) & \nodata & AGN & 0.59 \\
g793 & 44.924633 & 60.577140 & \nodata & \nodata & \nodata & 14.99(03) & 14.72(03) & 14.53(14) & 13.86(17) & \nodata & AGN & 0.73 \\
g794 & 44.925519 & 59.778182 & \nodata & \nodata & \nodata & 16.58(10) & 15.35(05) & 14.32(12) & 12.66(07) & \nodata & AGN & 0.00 \\
g795 & 44.928619 & 60.303375 & \nodata & \nodata & \nodata & 15.29(02) & 14.97(03) & 14.49(09) & 13.89(12) & \nodata & AGN & 0.27 \\
g796 & 44.936294 & 60.603379 & 16.27(14) & 15.49(16) & 14.91(15) & 14.50(04) & 14.41(06) & 14.06(10) & 13.02(13) & \nodata & AGN & 0.70 \\
g797 & 44.936595 & 60.029448 & \nodata & \nodata & \nodata & 15.00(03) & 14.30(02) & 13.45(06) & 12.48(05) & 8.40(09) & AGN & 0.04 \\
g798 & 44.937027 & 60.558791 & \nodata & \nodata & \nodata & 14.88(02) & 14.46(02) & 14.21(09) & 13.92(12) & \nodata & AGN & 0.79 \\
g799 & 44.944222 & 60.138525 & \nodata & \nodata & \nodata & 14.68(03) & 14.05(02) & 13.88(11) & 11.20(06) & 7.33(06) & PAH & 0.00 \\
g800 & 44.950218 & 60.621734 & \nodata & \nodata & \nodata & 14.74(02) & 14.57(03) & 14.46(12) & 13.56(13) & \nodata & AGN & 0.68 \\
g801 & 44.956781 & 59.595231 & \nodata & \nodata & \nodata & 15.46(03) & 14.65(03) & 14.34(12) & 11.56(04) & \nodata & PAH & 0.00 \\
g802 & 44.957212 & 60.587576 & \nodata & \nodata & \nodata & 15.37(03) & 15.11(04) & 14.44(13) & 13.78(16) & \nodata & AGN & 0.31 \\
g803 & 44.959444 & 59.833078 & \nodata & 15.95(12) & 15.68(18) & 14.78(03) & 14.67(03) & 13.72(12) & 11.12(02) & \nodata & PAH & 0.00 \\
g804 & 44.963957 & 59.987384 & \nodata & \nodata & \nodata & 14.43(01) & 13.66(01) & 13.18(05) & 10.79(02) & 7.35(09) & PAH & 0.00 \\
g805 & 44.969955 & 60.324801 & \nodata & \nodata & \nodata & 15.27(03) & 14.92(03) & 14.38(11) & 13.57(09) & \nodata & AGN & 0.25 \\
g806 & 44.970936 & 60.778782 & \nodata & \nodata & \nodata & 15.79(04) & 15.30(04) & 14.24(10) & 13.49(16) & \nodata & AGN & 0.01 \\
g807 & 44.972406 & 60.552398 & 16.34(12) & 15.38(12) & 14.87(14) & 14.36(02) & 14.12(02) & 14.12(09) & 13.61(16) & \nodata & AGN & 0.77 \\
g808 & 44.974078 & 60.573853 & \nodata & \nodata & \nodata & 15.25(03) & 15.07(04) & 15.07(17) & 13.41(10) & \nodata & PAH & 0.14 \\
g809 & 44.977698 & 60.188730 & \nodata & \nodata & \nodata & 15.29(02) & 14.91(03) & 14.38(10) & 12.94(06) & 8.88(10) & AGN & 0.06 \\
g810 & 44.983443 & 60.547507 & \nodata & \nodata & \nodata & 15.83(04) & 15.14(03) & 14.33(11) & 13.49(17) & 8.58(18) & AGN & 0.23 \\
g811 & 44.987171 & 60.562275 & \nodata & \nodata & \nodata & 15.37(03) & 15.00(03) & 14.27(10) & 13.74(16) & \nodata & AGN & 0.55 \\
g812 & 44.988181 & 60.583165 & \nodata & \nodata & \nodata & 14.47(02) & 13.95(02) & 13.50(07) & 12.45(08) & \nodata & AGN & 0.45 \\
g813 & 44.989693 & 60.410178 & \nodata & \nodata & \nodata & 15.33(03) & 14.88(03) & 14.41(10) & 13.63(10) & \nodata & AGN & 0.30 \\
g814 & 44.992069 & 60.115496 & \nodata & \nodata & \nodata & 15.38(03) & 14.43(02) & 13.60(09) & 12.66(11) & 8.82(09) & AGN & 0.07 \\
g815 & 44.994426 & 60.061197 & \nodata & \nodata & \nodata & 16.26(04) & 15.91(07) & 14.98(12) & 14.01(17) & \nodata & AGN & 0.00 \\
g816 & 44.995092 & 60.232136 & \nodata & \nodata & \nodata & 15.02(02) & 14.56(02) & 14.09(07) & 13.36(09) & \nodata & AGN & 0.33 \\
g817 & 44.997182 & 60.201773 & \nodata & \nodata & \nodata & 15.77(03) & 14.75(02) & 14.05(08) & 12.84(06) & \nodata & AGN & 0.07 \\
g818 & 45.002481 & 59.564342 & \nodata & \nodata & \nodata & 15.20(04) & 14.91(05) & 14.16(14) & 13.19(11) & \nodata & AGN & 0.21 \\
g819 & 45.006157 & 60.874344 & \nodata & \nodata & \nodata & 14.29(02) & 13.60(01) & 12.90(07) & 11.67(07) & 8.19(09) & AGN & 0.07 \\
g820 & 45.007462 & 60.568283 & \nodata & \nodata & \nodata & 14.79(02) & 14.44(03) & 14.11(08) & 13.81(14) & \nodata & AGN & 0.79 \\
g821 & 45.008808 & 60.781010 & \nodata & \nodata & \nodata & 15.58(04) & 14.79(03) & 14.04(09) & 12.66(09) & \nodata & AGN & 0.04 \\
g822 & 45.015455 & 60.787464 & \nodata & \nodata & \nodata & 15.46(03) & 14.83(03) & 13.95(12) & 13.20(19) & 9.17(10) & AGN & 0.19 \\
g823 & 45.015888 & 60.580414 & \nodata & \nodata & \nodata & 15.07(02) & 14.81(03) & 14.44(11) & 13.48(12) & 8.81(12) & AGN & 0.55 \\
g824 & 45.024372 & 60.346970 & 15.51(06) & 15.01(10) & 15.42(22) & 14.71(02) & 14.66(03) & 14.86(16) & 14.11(14) & \nodata & AGN & 0.34 \\
g825 & 45.031824 & 60.466190 & 16.52(16) & 15.66(16) & 15.15(19) & 14.80(02) & 14.56(02) & 14.18(10) & 13.31(10) & \nodata & AGN & 0.57 \\
g826 & 45.038191 & 60.734846 & \nodata & \nodata & \nodata & 15.15(02) & 14.69(02) & 14.52(11) & 13.43(10) & \nodata & AGN & 0.30 \\
g827 & 45.042624 & 60.556003 & \nodata & \nodata & \nodata & 14.53(02) & 14.01(02) & 13.38(06) & 12.54(06) & 8.41(07) & AGN & 0.71 \\
g828 & 45.054471 & 60.051994 & \nodata & \nodata & \nodata & 14.99(02) & 14.41(02) & 14.20(09) & 11.07(02) & 8.45(08) & PAH & 0.00 \\
g829 & 45.055838 & 60.596193 & \nodata & \nodata & \nodata & 15.20(03) & 14.46(03) & 13.88(08) & 12.87(08) & 8.97(16) & AGN & 0.50 \\
g830 & 45.060425 & 59.581208 & 14.52(03) & 14.02(03) & 13.82(04) & 13.82(01) & 13.82(02) & 13.66(15) & 11.56(03) & \nodata & PAH & 0.00 \\
g831 & 45.060627 & 60.528868 & 15.89(09) & 15.43(13) & 14.88(13) & 14.43(02) & 14.26(02) & 13.99(08) & 13.58(16) & \nodata & AGN & 0.63 \\
g832 & 45.078198 & 60.465395 & \nodata & \nodata & \nodata & 14.92(02) & 14.13(02) & 13.20(04) & 12.52(05) & 8.81(07) & AGN & 0.51 \\
g833 & 45.090443 & 60.941536 & \nodata & \nodata & \nodata & 14.71(02) & 14.40(03) & 13.94(13) & 12.97(14) & \nodata & AGN & 0.35 \\
g834 & 45.090709 & 60.584013 & \nodata & \nodata & \nodata & 15.38(03) & 14.94(03) & 14.38(10) & 13.85(16) & \nodata & AGN & 0.56 \\
g835 & 45.104939 & 60.479884 & \nodata & \nodata & \nodata & 15.04(02) & 14.64(02) & 14.31(10) & 13.87(11) & \nodata & AGN & 0.70 \\
g836 & 45.105377 & 60.449892 & 16.27(12) & 15.86(18) & 15.11(17) & 14.57(02) & 14.11(02) & 13.46(06) & 12.60(09) & 8.72(10) & AGN & 0.51 \\
g837 & 45.106828 & 60.274291 & \nodata & \nodata & \nodata & 14.96(02) & 13.92(01) & 12.95(04) & 11.77(02) & 7.64(04) & AGN & 0.04 \\
g838 & 45.117010 & 60.540226 & \nodata & \nodata & \nodata & 14.98(02) & 14.66(02) & 14.60(10) & 13.88(12) & \nodata & AGN & 0.70 \\
g839 & 45.117032 & 60.424755 & 16.47(15) & 15.47(14) & 15.07(17) & 14.61(02) & 14.53(02) & 14.46(12) & 13.70(19) & \nodata & AGN & 0.70 \\
g840 & 45.119307 & 59.684881 & 17.00(16) & 15.96(14) & \nodata & 14.95(02) & 14.24(02) & 13.64(10) & 12.61(06) & \nodata & AGN & 0.27 \\
g841 & 45.120393 & 60.650492 & 14.77(04) & 14.17(05) & 14.16(07) & 14.01(01) & 14.03(01) & 13.91(09) & 13.50(09) & \nodata & AGN & 0.44 \\
g842 & 45.126854 & 60.838266 & 16.77(19) & 15.90(19) & 15.26(18) & 15.04(02) & 14.92(04) & 14.83(17) & 12.85(14) & \nodata & PAH & 0.00 \\
g843 & 45.129363 & 60.408429 & 17.05(23) & 15.72(16) & 15.26(19) & 14.76(02) & 14.40(02) & 14.24(08) & 13.60(19) & \nodata & AGN & 0.61 \\
g844 & 45.145106 & 60.666468 & 15.18(05) & 14.35(06) & 14.18(07) & 14.10(01) & 14.07(01) & 14.11(08) & 13.55(10) & \nodata & AGN & 0.36 \\
g845 & 45.145721 & 60.456175 & 15.98(10) & 15.03(09) & 14.98(15) & 14.56(02) & 14.54(03) & 14.29(08) & 13.98(13) & \nodata & AGN & 0.72 \\
g846 & 45.148176 & 60.328733 & 15.41(06) & 14.93(09) & 14.67(12) & 14.67(02) & 14.60(02) & 14.69(11) & 13.95(16) & \nodata & AGN & 0.34 \\
g847 & 45.148999 & 60.998389 & 15.12(05) & \nodata & 14.20(08) & 14.05(01) & 13.99(02) & 13.96(17) & 12.61(16) & \nodata & PAH & 0.33 \\
g848 & 45.149179 & 60.717709 & 16.43(13) & 15.61(14) & 14.96(14) & 14.68(02) & 14.48(02) & 14.30(11) & 13.82(11) & 10.31(33) & AGN & 0.37 \\
g849 & 45.149616 & 60.412319 & \nodata & \nodata & \nodata & 15.26(03) & 14.88(04) & 14.72(13) & 14.00(15) & \nodata & AGN & 0.58 \\
g850 & 45.158172 & 60.381597 & \nodata & \nodata & \nodata & 15.84(04) & 15.19(04) & 15.03(18) & 13.51(18) & \nodata & PAH & 0.00 \\
g851 & 45.162154 & 60.682630 & 16.13(10) & 15.10(09) & 15.06(16) & 14.55(01) & 14.46(02) & 14.43(10) & 13.90(11) & \nodata & AGN & 0.36 \\
g852 & 45.163150 & 60.544080 & \nodata & \nodata & \nodata & 14.91(02) & 14.68(02) & 14.46(10) & 13.74(20) & 9.63(19) & AGN & 0.70 \\
g853 & 45.165030 & 60.493626 & \nodata & \nodata & \nodata & 14.94(02) & 14.65(02) & 14.18(08) & 12.20(04) & 10.38(40) & PAH & 0.00 \\
g854 & 45.167791 & 60.476472 & \nodata & \nodata & \nodata & 15.09(02) & 14.73(02) & 14.10(10) & 13.69(16) & \nodata & AGN & 0.68 \\
g855 & 45.169539 & 60.540365 & 15.75(07) & 14.67(07) & 14.45(09) & 14.25(01) & 14.31(02) & 14.20(09) & 13.55(12) & \nodata & AGN & 0.77 \\
g856 & 45.172853 & 60.560433 & \nodata & \nodata & \nodata & 15.47(02) & 15.04(03) & 14.91(11) & 14.18(18) & \nodata & AGN & 0.32 \\
g857 & 45.187007 & 60.489382 & \nodata & \nodata & \nodata & 15.07(02) & 14.97(03) & 14.53(12) & 13.17(11) & \nodata & PAH & 0.00 \\
g858 & 45.192776 & 60.514868 & 16.52(14) & 15.47(14) & 15.22(18) & 14.69(02) & 14.47(02) & 14.35(10) & 13.84(17) & \nodata & AGN & 0.79 \\
g859 & 45.199453 & 60.521866 & \nodata & \nodata & \nodata & 15.63(05) & 15.19(05) & 14.36(11) & 13.95(12) & \nodata & AGN & 0.33 \\
g860 & 45.206862 & 59.584306 & 17.06(17) & 15.99(12) & 15.22(12) & 14.47(02) & 14.05(02) & 14.04(11) & 11.23(03) & \nodata & PAH & 0.00 \\
g861 & 45.207558 & 60.474355 & \nodata & \nodata & \nodata & 15.48(04) & 15.26(04) & 14.88(11) & 13.66(16) & \nodata & AGN & 0.08 \\
g862 & 45.210502 & 60.521592 & \nodata & 15.64(16) & \nodata & 15.11(02) & 14.79(03) & 14.28(10) & 13.57(09) & \nodata & AGN & 0.59 \\
g863 & 45.222893 & 60.522242 & \nodata & \nodata & \nodata & 15.37(02) & 14.85(03) & 14.31(10) & 13.58(11) & \nodata & AGN & 0.55 \\
g864 & 45.224932 & 60.149929 & \nodata & \nodata & \nodata & 15.05(04) & 14.20(02) & 13.36(09) & 12.43(19) & 8.75(11) & AGN & 0.04 \\
g865 & 45.227003 & 60.510474 & 15.16(05) & 14.57(06) & 14.48(09) & 14.38(01) & 14.39(02) & 14.31(09) & 13.81(14) & \nodata & AGN & 0.79 \\
g866 & 45.227387 & 60.709728 & 15.55(07) & 15.37(12) & 15.24(18) & 14.87(02) & 14.82(03) & 14.74(12) & 13.65(13) & \nodata & PAH & 0.00 \\
g867 & 45.227827 & 60.476416 & \nodata & \nodata & \nodata & 15.20(04) & 14.87(04) & 14.91(16) & 13.88(10) & \nodata & PAH & 0.00 \\
g868 & 45.228932 & 60.422175 & \nodata & \nodata & \nodata & 15.95(07) & 15.22(06) & 14.60(10) & 13.65(12) & \nodata & AGN & 0.18 \\
g869 & 45.230627 & 60.756310 & 16.78(20) & \nodata & 14.85(14) & 14.10(01) & 13.44(01) & 11.92(02) & 9.89(02) & 6.09(05) & PAH & 0.00 \\
g870 & 45.239003 & 60.480119 & \nodata & \nodata & \nodata & 15.52(05) & 14.86(04) & 14.27(09) & 13.05(11) & 10.05(40) & AGN & 0.15 \\
g871 & 45.244919 & 60.530695 & \nodata & \nodata & \nodata & 15.31(04) & 14.60(04) & 14.20(08) & 12.24(04) & 8.82(17) & PAH & 0.00 \\
g872 & 45.245134 & 60.504533 & \nodata & \nodata & \nodata & 16.49(07) & 15.39(04) & 14.45(13) & 13.15(16) & \nodata & AGN & 0.02 \\
g873 & 45.248845 & 60.764554 & \nodata & \nodata & \nodata & 14.37(02) & 14.21(03) & 13.90(10) & 11.76(07) & \nodata & PAH & 0.00 \\
g874 & 45.249874 & 60.466950 & \nodata & \nodata & \nodata & 15.37(02) & 15.35(04) & 15.29(18) & 14.34(18) & \nodata & AGN & 0.12 \\
g875 & 45.250267 & 60.539558 & \nodata & \nodata & \nodata & 14.69(04) & 14.61(03) & 14.63(16) & 14.10(19) & \nodata & AGN & 0.76 \\
g876 & 45.251095 & 60.459819 & 16.44(14) & 15.74(17) & 15.00(15) & 14.96(02) & 14.90(02) & 14.57(09) & 13.70(10) & \nodata & AGN & 0.56 \\
g877 & 45.257366 & 60.455621 & \nodata & \nodata & \nodata & 15.59(03) & 15.01(03) & 14.60(11) & 12.70(04) & 9.47(14) & PAH & 0.00 \\
g878 & 45.259501 & 60.374909 & \nodata & \nodata & \nodata & 15.85(03) & 14.76(02) & 13.81(05) & 12.71(04) & 8.76(07) & AGN & 0.05 \\
g879 & 45.275312 & 60.507694 & \nodata & \nodata & \nodata & 14.78(02) & 14.25(02) & 13.92(07) & 12.87(06) & 8.79(20) & AGN & 0.70 \\
g880 & 45.277039 & 59.859335 & \nodata & \nodata & \nodata & 14.92(03) & 14.01(02) & 13.24(07) & 11.82(04) & \nodata & AGN & 0.06 \\
g881 & 45.277601 & 60.411965 & \nodata & \nodata & \nodata & 14.92(02) & 14.43(02) & 14.35(09) & 13.78(17) & \nodata & AGN & 0.63 \\
g882 & 45.278474 & 60.531866 & \nodata & \nodata & \nodata & 14.78(06) & 14.08(03) & 13.16(05) & 12.59(08) & \nodata & AGN & 0.71 \\
g883 & 45.278872 & 60.613420 & \nodata & \nodata & \nodata & 15.00(02) & 14.65(02) & 14.05(08) & 13.58(15) & \nodata & AGN & 0.39 \\
g884 & 45.281572 & 60.515698 & \nodata & \nodata & \nodata & 15.01(02) & 14.55(02) & 14.02(06) & 13.73(10) & \nodata & AGN & 0.73 \\
g885 & 45.284539 & 59.627184 & \nodata & \nodata & \nodata & 15.26(03) & 14.06(02) & 13.48(08) & 12.32(06) & \nodata & AGN & 0.27 \\
g886 & 45.290094 & 60.481853 & \nodata & \nodata & \nodata & 15.65(04) & 14.82(04) & 13.92(06) & 12.76(06) & 9.02(22) & AGN & 0.09 \\
g887 & 45.296264 & 60.519130 & 16.03(09) & 15.25(11) & \nodata & 14.43(01) & 14.31(02) & 14.06(08) & 13.72(15) & \nodata & AGN & 0.79 \\
g888 & 45.296455 & 60.648707 & 16.87(19) & 15.85(18) & 15.18(16) & 14.67(02) & 14.36(02) & 13.78(07) & 12.74(09) & 8.94(11) & AGN & 0.29 \\
g889 & 45.310226 & 60.472826 & 16.00(09) & 15.10(09) & 14.59(11) & 14.28(01) & 14.10(02) & 13.87(08) & 12.51(05) & \nodata & PAH & 0.00 \\
g890 & 45.311660 & 60.523661 & \nodata & \nodata & \nodata & 15.61(02) & 14.84(02) & 13.99(07) & 13.39(07) & \nodata & AGN & 0.55 \\
g891 & 45.317933 & 60.477771 & \nodata & 15.46(14) & \nodata & 14.83(02) & 14.57(02) & 14.02(08) & 13.10(09) & \nodata & AGN & 0.64 \\
g892 & 45.326300 & 60.483113 & \nodata & \nodata & \nodata & 14.84(02) & 14.06(03) & 13.24(09) & 12.36(09) & \nodata & AGN & 0.51 \\
g893 & 45.328900 & 60.524661 & \nodata & \nodata & \nodata & 15.33(02) & 14.95(03) & 14.52(12) & 13.66(10) & \nodata & AGN & 0.55 \\
g894 & 45.337911 & 60.453999 & \nodata & \nodata & \nodata & 15.87(03) & 15.53(03) & 15.01(17) & 13.88(18) & \nodata & AGN & 0.00 \\
g895 & 45.348450 & 60.635879 & 16.70(17) & 15.74(16) & 15.21(16) & 14.62(01) & 14.31(02) & 14.09(08) & 13.76(12) & \nodata & AGN & 0.37 \\
g896 & 45.350622 & 60.740457 & 14.29(03) & 13.69(05) & 13.47(05) & 13.38(01) & 13.41(01) & 13.39(13) & 12.12(05) & \nodata & PAH & 0.35 \\
g897 & 45.354511 & 60.544654 & 16.51(14) & 15.87(18) & 15.22(15) & 14.86(03) & 14.63(03) & 14.07(08) & 13.08(07) & \nodata & AGN & 0.40 \\
g898 & 45.368164 & 60.721700 & 14.57(04) & 14.03(05) & 13.75(04) & 13.61(01) & 13.64(01) & 12.95(07) & 11.59(10) & \nodata & PAH & 0.00 \\
g899 & 45.382905 & 60.439440 & 16.87(18) & 15.46(13) & 14.79(10) & 13.77(02) & 13.21(01) & 12.86(12) & 11.45(08) & \nodata & PAH & 0.00 \\
g900 & 45.414077 & 60.607395 & 15.61(08) & \nodata & 14.54(10) & 14.38(02) & 14.40(02) & 14.18(10) & 13.87(18) & \nodata & AGN & 0.37 \\
g901 & 45.429501 & 60.103696 & \nodata & \nodata & \nodata & 15.31(03) & 15.09(04) & 14.60(16) & 13.23(12) & \nodata & AGN & 0.04 \\
g902 & 45.444418 & 60.123599 & \nodata & \nodata & \nodata & 15.49(03) & 15.22(04) & 14.70(17) & 12.27(06) & 8.19(06) & PAH & 0.00 \\
g903 & 45.463813 & 60.250334 & \nodata & \nodata & \nodata & 14.21(02) & 13.88(03) & 13.55(06) & 11.75(06) & 9.03(15) & PAH & 0.00 \\
g904 & 45.489523 & 60.744982 & 15.96(07) & 15.07(09) & 14.84(11) & 14.59(02) & 14.48(02) & 14.19(11) & 13.68(20) & \nodata & AGN & 0.08 \\
g905 & 45.561236 & 60.709705 & \nodata & 15.33(14) & 14.27(10) & 13.46(02) & 13.07(01) & 12.70(07) & 10.92(07) & 7.79(09) & PAH & 0.00 \\
g906 & 45.563996 & 60.762994 & \nodata & \nodata & \nodata & 16.09(06) & 15.24(05) & 14.43(14) & 13.40(12) & \nodata & AGN & 0.01 \\
g907 & 45.572060 & 60.291529 & 15.33(06) & 14.67(07) & 14.44(09) & 14.27(01) & 14.30(02) & 14.42(11) & 13.72(19) & \nodata & AGN & 0.10 \\
g908 & 45.598429 & 60.457383 & \nodata & \nodata & \nodata & 15.69(04) & 14.86(03) & 15.01(20) & 12.03(07) & 8.56(11) & PAH & 0.00 \\
g909 & 45.634698 & 60.478368 & \nodata & \nodata & \nodata & 15.27(04) & 14.34(03) & 13.56(11) & 12.40(17) & \nodata & AGN & 0.02 \\
g910 & 45.635183 & 60.743577 & \nodata & \nodata & \nodata & 15.15(03) & 13.68(01) & 12.53(03) & 11.50(05) & \nodata & AGN & 0.02 \\
g911 & 45.681028 & 60.708658 & \nodata & \nodata & \nodata & 15.85(05) & 14.82(03) & 13.93(11) & 12.82(18) & \nodata & AGN & 0.03 \\
g912 & 45.697807 & 60.459186 & \nodata & \nodata & \nodata & 16.03(13) & 13.79(06) & 12.48(09) & 11.47(09) & \nodata & AGN & 0.01 \\
g913 & 45.729590 & 60.652368 & 16.34(14) & 15.36(13) & 14.44(09) & 13.35(01) & 12.85(01) & 11.66(02) & 9.22(01) & \nodata & PAH & 0.00 \\
g914 & 45.735771 & 60.652317 & \nodata & \nodata & \nodata & 14.98(04) & 14.84(03) & 13.93(13) & 11.72(11) & \nodata & PAH & 0.00 \\
g915 & 45.757865 & 60.299835 & \nodata & \nodata & \nodata & 15.23(02) & 15.18(04) & 14.80(17) & 13.71(18) & \nodata & AGN & 0.12 \\
g916 & 45.767659 & 60.414424 & 16.49(15) & 15.69(15) & 14.91(12) & 14.01(02) & 13.65(02) & 12.93(12) & 11.77(20) & \nodata & AGN & 0.07 \\
g917 & 45.780794 & 60.748240 & 15.56(06) & 14.65(07) & 14.41(08) & 14.13(03) & 14.20(03) & 14.27(14) & 13.65(13) & \nodata & AGN & 0.18 \\
g918 & 45.791322 & 60.333443 & \nodata & \nodata & \nodata & 14.90(03) & 14.48(03) & 13.91(12) & 12.75(09) & \nodata & AGN & 0.21 \\
g919 & 45.818804 & 60.282245 & \nodata & \nodata & \nodata & 14.86(02) & 14.50(02) & 14.12(09) & 12.78(04) & \nodata & AGN & 0.05 \\
g920 & 45.832097 & 60.279550 & \nodata & 15.45(12) & 15.10(14) & 14.77(02) & 14.73(03) & 14.47(14) & 14.12(14) & \nodata & AGN & 0.17 \\
g921 & 45.839754 & 60.518591 & \nodata & \nodata & \nodata & 14.30(08) & 14.45(10) & 11.35(10) & 9.59(11) & \nodata & PAH & 0.13 \\
g922 & 45.869995 & 60.648191 & \nodata & \nodata & \nodata & 14.59(05) & 13.70(02) & 12.99(16) & 11.82(15) & \nodata & AGN & 0.09 \\
g923 & 45.939262 & 60.413851 & \nodata & \nodata & \nodata & 14.85(02) & 14.15(02) & 13.49(10) & 12.33(15) & \nodata & AGN & 0.08 \\
g924 & 45.960475 & 60.593318 & \nodata & \nodata & \nodata & 14.59(02) & 14.02(02) & 13.57(09) & 12.49(08) & \nodata & AGN & 0.27 \\
g925 & 45.979907 & 60.455308 & 16.77(17) & 15.60(13) & 15.42(20) & 14.77(02) & 14.55(02) & 14.09(13) & 13.21(17) & \nodata & AGN & 0.15 \\
g926 & 45.990611 & 60.423176 & \nodata & \nodata & \nodata & 14.68(02) & 13.93(02) & 13.21(04) & 12.51(06) & \nodata & AGN & 0.06 \\
g927 & 45.999560 & 60.410705 & \nodata & \nodata & \nodata & 15.92(04) & 15.12(04) & 13.89(10) & 12.75(08) & \nodata & AGN & 0.00 
\enddata
\tablecomments{Values in parentheses signify error in last 2 digits of magnitude value. Right ascension and Declination coordinates are J2000.0.} 
\tablenotetext{a}{Galaxy type: AGN or `PAH galaxy' as defined in text.}
\tablenotetext{b}{Probability that source is a YSO based on local space density, color, magnitude criteria: see text.}
\end{deluxetable}

